Online and Fully-Dynamic Sorting

Online sorting asks how to place $n$ sequentially arriving elements in an array to minimize the sum of absolute differences between consecutive elements. Fully-dynamic sorting further extends the problem to allow both element insertions and deletions. Without recourse, these problems face strong lower bounds on the competitive ratio: $\Omega(\sqrt{n})$ for online sorting and $\Omega(n)$ for fully-dynamic sorting. In sharp contrast, we show that allowing only poly-logarithmic recourse yields at least exponential improvements in the competitive ratio for both problems:(1) Our main algorithmic result is a deterministic fully-dynamic sorting algorithm that is $O(\log^2 n)$-competitive and has $O(\log^4 n)$ amortized recourse per update. We complement this with a lower bound showing that any deterministic algorithm with any $O(\mathrm{polylog}(n))$ competitive ratio has amortized recourse at least $\Omega(\sqrt{\log n})$.(2) For the insertion-only setting, we establish a family of approximation--recourse tradeoffs, including $O(\log\log n)$ competitive ratio with $O(\log\log n)$ amortized recourse. Given the lower bound in the fully-dynamic case, this result shows that the insertion-only problem yields exponentially better bounds than the fully-dynamic one.(3) Finally, we show that the stronger approximation-recourse tradeoff for the insertion-only case extends to the fully-dynamic setting when the array has $(1+\varepsilon)n$ space.

==> DST_onelevel.tex <==
First, we assume that after any deletion, an insertion follows; otherwise, we ignore the deletion operation, as it does not increase the cost.
We also assume that, at the beginning of the algorithm's run, the array is sorted. \ov{Need to see how we can smooth this assumption out later on.}
Before defining the update logic, we establish a structural partition of the array into two distinct regions, which we refer to as the \emph{Old} and the \emph{New} sections.

\begin{itemize}
    \item The \emph{Old} section: This part of the array contains the elements that were present before the last time the array was completely sorted. It is divided into $m = \sqrt{n}$ blocks, each initially of size $\sqrt{n}$. The \emph{Old} section is the primary workspace for the Ripple algorithm.
    \item The \emph{New} Section: This part contains elements that were inserted after the last time the array was completely sorted. It is maintained as a single, contiguous sorted sub-array of size at most $\sqrt{n}$.
\end{itemize}

To ensure the integrity of this separation, every insertion is handled by the following redirection rule:
Suppose a new element $x$ is inserted at a position $i$ that falls within the old section, We:

We identify the element currently sitting at the boundary between the Old section and the New section, denoted as $y_{boundary}$. We swap the newly inserted element $x$ with $y_{boundary}$. As a result of this single operation:
\begin{itemize}
    \item The new element $x$ is transferred directly into the New section (at the boundary position), where its final placement is handled by the balancing algorithm of the new section.
    \item The extreme element $y_{boundary}$ (the maximum or minimum of the Old section, depending on $\sigma$) is now physically located at position $p$ within block $B_k$.
\end{itemize}
We refer to this operation as the \textbf{Boundary Swap}.
If an element $x$ is inserted into the new section, it is handled by the balancing algorithm for the section directly.

The array is physically organized such that the Old section and the New section are contiguous.

To support both forward and backward flows using a single unified procedure, we define a direction parameter $\sigma \in \{1, -1\}$. The algorithm relies on the topological boundary between the Old section and the New section:
\begin{itemize}
    \item \textbf{Forward Flow ($\sigma = 1$):} The New section is located after the Old section. The boundary element is the last element of the Old section, which corresponds to the \textit{largest} value in the Old section. The target terminal block is the final block, $B_{\sqrt{n}}$.
    \item \textbf{Backward Flow ($\sigma = -1$):} The New section is located before the Old section. The boundary element is the first element of the Old section, which corresponds to the \textit{smallest} value in the Old section. The target terminal block is the first block, $B_1$.
\end{itemize}

\subsubsection{Balancing of the New Section}

For any new element that is inserted, we simply always completely sort the section.
Therefore, it is always maintained as sorted.

\subsubsection{Balancing of the Old Section}

When a new element $x$ is inserted at a position $p$ that falls within the Old section (let $B_k$ be the block containing position $p$), the algorithm executes the following two phases.


\paragraph{Phase 1: Local Shift}
The element $y_{boundary}$ must be aligned with the internal structure of block $B_k$. Through a series of local swaps within $B_k$, we move $y_{boundary}$ from position $p$ strictly to the boundary between the Origin section ($O_k$) and the Transfer section ($T_k$).

\paragraph{Phase 2: The Ripple to the Terminal Block}
Because $y_{boundary}$ represents an extreme value for the entire Old section, its correct semantic destination is the terminal block of the flow ($B_{\sqrt{n}}$ if $\sigma = 1$, or $B_1$ if $\sigma = -1$). We use the ripple procedure to propagate it to its final destination:
\begin{enumerate}
    \item Starting from its position at the $O_k/T_k$ boundary in block $B_k$, $y_{boundary}$ is swapped with the element at the exit boundary of $B_k$.
    \item The displaced element crosses the block boundary into the adjacent block $B_{k+\sigma}$, entering its Transfer section.
    \item This cascaded swapping continues sequentially through the adjacent blocks until the ripple reaches the terminal block.
    \item In the terminal block, $y_{boundary}$ is shifted to the absolute extreme end of the block (the very end if $\sigma=1$, or the very beginning if $\sigma=-1$).
\end{enumerate}

\subsubsection{Structural Invariants}

The algorithm maintains the following four invariants throughout its execution. These are restored at the end of every insertion-deletion pair.

\begin{enumerate}
    \item \textbf{Block Monotonicity:} 
    For any two adjacent blocks $B_i$ and $B_{i+1}$ in the Old section, the values are ordered such that:
    \[ \max(B_i) \leq \min(B_{i+1}) \]
    This ensures that despite internal movement, the blocks remain ordered relative to one another.

    \item \textbf{Internal Block Order:} 
    Within each block $B_i$, the Origin section ($O_i$) and the Transfer section ($T_i$) are both internally sorted. Their relative position depends on the flow direction $\sigma$:
    \begin{itemize}
        \item If $\sigma = 1$ (Forward), then $O_i < T_i$.
        \item If $\sigma = -1$ (Backward), then $T_i < O_i$.
    \end{itemize}

    \item \textbf{Transfer Identity:}
    The elements in the Transfer section $T_k$ of block $B_k$ consist exclusively of elements that were passed from the immediate preceding block in the flow ($B_{k-\sigma}$) during the current operation.

    \item \textbf{Block Size:}
    Let $B_{term}$ be the terminal block of the flow ($B_{\sqrt{n}}$ if $\sigma = 1$, or $B_1$ if $\sigma = -1$). Because one element is ceded to the New section during the boundary swap of each operation, the sizes of the blocks are maintained as follows:
    \begin{itemize}
        \item For every non-terminal block $i \neq term$, the total size remains strictly constant: $|O_i| + |T_i| = \sqrt{n}$.
        \item For the terminal block $B_{term}$, its total size strictly reduces by one element during each operation in the old section.
    \end{itemize}
\end{enumerate}
We prove critical claims in order to bound the recourse and cost used by the algorithm.
\begin{claim}
    \label{cl:constant-capacity}
    For any non-terminal block $B_i$ in the flow, the total number of elements remains exactly $\sqrt{n}$ after every operation.
\end{claim}
\begin{proof}
    We prove this by tracking the net change in the number of elements for any non-terminal block $B_i$ during a single operation. Every block in the Old section starts exactly $\sqrt{n}$ elements. We must show that the three phases of the update operation contribute a net size change of exactly zero to any $B_i \neq B_{term}$.
    
    \begin{itemize}
        \item \textbf{The Boundary Swap}: If the newly inserted element $x$ is positioned within $B_i$, the algorithm swaps $x$ with the extreme boundary element of the Old section, $y_{boundary}$. Because $x$ exits the block (moving to the New section) and $y_{boundary}$ enters the block, the net change in the size of $B_i$ is $+1 - 1 = 0$. If the insertion occurs in a different block, $B_i$ is unaffected by this phase.
        
        \item \textbf{Phase 1 (Local Boundary Shift):} This phase consists entirely of internal swaps designed to correctly position $y_{boundary}$ at the boundary between $O_i$ and $T_i$. Since all movement is strictly inside a block, no elements enter or leave $B_i$. The net change is $0$.
        
        \item \textbf{Phase 2 (The Ripple):} If $B_i$ lies on the propagation path, it participates in a cascading sequence of swaps. Specifically, $B_i$ receives exactly one element from the preceding block ($B_{i-\sigma}$) at its entry boundary, and concurrently ejects exactly one element from its exit boundary into the succeeding block ($B_{i+\sigma}$). If $B_i$ is not on the ripple path, it is not involved, and thus the net change is $0$.
    \end{itemize}
\end{proof}

\begin{claim}
    \label{cl:terminal-capacity}
    For the terminal block $B_{term}$, the total size strictly decreases by one element per operation.
\end{claim}
\begin{proof}
    During Phase 1 (The Boundary Swap), the algorithm identifies $y_{boundary}$, which physically resides at the extreme end of $B_{term}$ (the very end if $\sigma=1$, or the very beginning if $\sigma=-1$). The newly inserted element $x$ is swapped into this boundary position, and this position is immediately ceded to the New section. As a result, the size of the old section strictly decreases by exactly one slot. 
    By \cref{cl:constant-capacity}, the sum of the sizes of all non-terminal blocks remains unchanged. Therefore, the size of $B_{term}$ strictly decreases by exactly one element per operation.
\end{proof}

\begin{claim}
    \label{cl:never-empty}
    No block in the old section ever becomes empty during the $\sqrt{n}$ operations between global sorts.
\end{claim}
\begin{proof}
    Following a global sort, every block initializes with exactly $\sqrt{n}$ elements. By \cref{cl:constant-capacity}, all non-terminal blocks strictly maintain this size. By \cref{cl:terminal-capacity}, the terminal block loses exactly one element per operation. Because a global reset occurs every $\sqrt{n}$ operations, the terminal block's size decreases from $\sqrt{n}$ to a minimum of $\sqrt{n} - \sqrt{n} = 0$, when a sort operation occurs.
\end{proof}

\begin{corollary}
    By the combined results of \cref{cl:constant-capacity}, \cref{cl:terminal-capacity}, and \cref{cl:never-empty}, the structure strictly satisfies the Block Size Invariant.
\end{corollary}

\begin{claim}
    \label{cl:transfer-origin}
    During an operation with flow direction $\sigma$, the elements entering the transfer section $T_k$ of block $B_k$ originate exclusively from the adjacent block $B_{k-\sigma}$.
\end{claim}
\begin{proof}
    By the definition of the ripple procedure, the element that enters the transfer section $T_k$ of block $B_k$ is drawn directly from the origin section of the adjacent preceding block, $B_{k-\sigma}$. 
    Because \cref{cl:never-empty} guarantees that the sections never empty during the operations between global sorts, the origin section of $B_{k-\sigma}$ always contains at least one element available to be swapped.
\end{proof}

\begin{corollary}
    Because elements enter the transfer sections exclusively from adjacent blocks (\cref{cl:transfer-origin}) and consist solely of the extreme boundary element propagating through the flow, the algorithm satisfies the Transfer Identity Invariant.
\end{corollary}


\begin{claim}
    \label{cl:internal-sections-sorted}
    Within each block $B_i$, both the origin section $O_i$ and the transfer section $T_i$ are internally completely sorted.
\end{claim}
\begin{proof}
    We proceed by induction on the sequence of operations since the last global sort. 
    
    \textbf{Base Case:} Immediately following a global sort, the entire Old section is completely sorted. For every block $B_i$, the transfer section $T_i$ is initialized as empty (which is trivially sorted).
    
    \textbf{Inductive Step:} Assume $O_i$ and $T_i$ are internally sorted prior to an insertion-deletion pair. We examine the effects of both the deletion and the insertion phases on their internal structures:
    
    \begin{itemize}
        \item \textbf{Handling the Deletion Step:} If the specified element to be deleted resides within block $B_i$ (whether it belongs to $O_i$ or $T_i$). The algorithm resolves this by performing a shift of the remaining elements in that section such that the the new element is on the boundary between the transfer and origin sections. The shift preserves the relative order of all shifted elements, and the invariant as a result.
        
      \item \textbf{Handling the Ripple in $O_i$:} During Phase 2 (The Ripple), as the cascading swaps propagate through $B_i$, the origin section $O_i$ actively cedes an element from its boundary to the transfer section of the adjacent block ($T_{i+\sigma}$). Because $O_i$ strictly loses an element during this phase, and removing an element from a sorted sequence trivially preserves the monotonic order of the remaining elements, $O_i$ remains completely sorted.
        
        \item \textbf{Handling the Ripple in $T_i$:} The transfer section $T_i$ is modified during Phase 2, receiving an element from $B_{i-\sigma}$ and yielding an element to $B_{i+\sigma}$. Because these swaps occur at the boundaries of $T_i$, the section acts as a contiguous shift buffer. The relative internal order of the elements already inside $T_i$ is perfectly preserved. Moreover, the sequence of elements entering $T_i$ over consecutive operations consists exactly of the extreme boundary elements ($y_{boundary}$). Because we process the extremes sequentially, this incoming sequence is monotonic and remains completely sorted.
    \end{itemize}
\end{proof}

\begin{claim}
    \label{cl:internal-relative-order}
    The relative ordering of sections within a block $B_i$ strictly respects the flow direction $\sigma$: if $\sigma = 1$, then $O_i < T_i$; if $\sigma = -1$, then $T_i < O_i$.
\end{claim}
\begin{proof}
    We evaluate the relative values of the elements in $O_i$ and $T_i$ based on the identity of the elements that populate the transfer section during an operation.
    
    The transfer section $T_i$ is populated exclusively by the extreme boundary element, $y_{boundary}$, as it propagates through the block to its terminal destination. 
    
    By the algorithm's definition, the flow direction $\sigma$ determines the extreme element. When $\sigma = 1$, $y_{boundary}$ is the global maximum of the old section, making it strictly greater than any comparatively bounded native element in $O_i$, thus yielding $O_i < T_i$. Conversely, when $\sigma = -1$, $y_{boundary}$ is the global minimum of the old section, making it strictly less than any native element in $O_i$, thus yielding $T_i < O_i$. 
    
    Because $T_i$ only ever contains this extreme element passing through, this relative ordering is preserved throughout the operation.
\end{proof}

\begin{corollary}
    By the combined results of \cref{cl:internal-sections-sorted} and \cref{cl:internal-relative-order}, the structure satisfies the Internal Block Order Invariant (Invariant 2).
\end{corollary}

\begin{claim}
    \label{cl:global-monotonicity}
    For any two adjacent blocks $B_i$ and $B_{i+1}$ in the old section, the global monotonicity $\max(B_i) \leq \min(B_{i+1})$ holds after every operation.
\end{claim}
\begin{proof}
    We proceed by induction on the sequence of operations. Following a global sort, the old section is completely sorted, so $\max(B_i) \leq \min(B_{i+1})$ holds trivially for all adjacent blocks. 
    
    During any update operation, internal deletions strictly create a subset of the block's elements, that cannot violate existing bounds. During the insertion ripple (Phase 2), elements only cross boundaries in two specific ways:
    \begin{itemize}
        \item If $\sigma = 1$ (Forward Flow), block $B_i$ passes its strict maximum element to $B_{i+1}$.
        \item If $\sigma = -1$ (Backward Flow), block $B_{i+1}$ passes its strict minimum element to $B_i$.
    \end{itemize}
    Because the blocks are internally sorted (\cref{cl:internal-sections-sorted}) and were globally monotonic prior to the swap, moving the maximum of a "smaller" block to a "larger" block, or the minimum of a "larger" block to a "smaller" block, trivially preserves the global monotonicity $\max(B_i) \leq \min(B_{i+1})$.
\end{proof}
\begin{corollary}
    By \cref{cl:global-monotonicity}, the structure strictly satisfies the Block Monotonicity Invariant (Invariant 1).
\end{corollary}

\subsubsection{Recourse Bound}

\begin{theorem}
    The amortized recourse of the algorithm per update operation is $O(\sqrt{n})$.
\end{theorem}
\begin{proof}
    We account for the recourse used across the distinct phases of the algorithm. During a single insertion-deletion pair, the algorithm incurs the following worst-case recourse costs:
    \begin{itemize}
        \item \textbf{Maintaining the new section}: The New section holds at most $\sqrt{n}$ elements. Inserting an element and maintaining its internal sorted order via a shift requires at most $O(\sqrt{n})$ recourse.
        \item \textbf{Boundary shift:} Replacing the last element with the newly inserted element takes exactly 1 swap.
        \item \textbf{Local boundary shift:} Moving the boundary element $y_{boundary}$ to the edge of the transfer section $T_i$ requires a shift of the elements. Since the block size is at most $\sqrt{n}$, this costs at most $O(\sqrt{n})$.
        \item \textbf{The Ripple:} Propagating $y_{boundary}$ through the transfer sections requires exactly one swap per block boundary. Because there are at most $\sqrt{n}$ blocks in the Old section, the inter-block cascading swaps cost exactly $O(\sqrt{n})$.
    \end{itemize}
    Summing the strictly local operations yields a worst-case recourse of $O(\sqrt{n})$ per step. 
    
    Finally, the algorithm performs a complete global sort of all $n$ elements exactly once every $\sqrt{n}$ operations. This imposes a worst-case recourse of $O(n)$ at the epoch boundary. Amortized over the $\sqrt{n}$ operations of the epoch, the global rebuild contributes $\frac{O(n)}{\sqrt{n}} = O(\sqrt{n})$ to the per-step cost. 
    
    Therefore, the total amortized recourse per operation is bounded by $O(\sqrt{n})$.
\end{proof}

\subsubsection{Cost Bound}

\begin{theorem}
    The algorithm is $O(1)$-competitive.
\end{theorem}
\begin{proof}
    At any given step, let $A$ be the current set of elements maintained by the algorithm. The optimal offline adversary must arrange these elements in perfectly sorted order. The minimum possible cost is \[ OPT = \max(A) - \min(A) \].
    
    We evaluate the cost of our algorithm's configuration, $ALG$. The total variation of any array can be bounded by the sum of its "drops" (decreasing steps where $A[j] > A[j+1]$) plus the total increasing value. Specifically, $ALG \le 2 \sum (\text{drops}) + (\max(A) - \min(A))$.
    
    We locate all possible drops in the algorithm's structure:
    \begin{itemize}
        \item By \cref{cl:internal-sections-sorted}, both $O_i$ and $T_i$ of every block are internally completely sorted. No drops occur inside these sections.
        \item By \cref{cl:global-monotonicity}, adjacent blocks maintain global monotonicity ($\max(B_i) \leq \min(B_{i+1})$). The transition across the boundary from one block to the next contributes zero drops.
        \item The new section is maintained in sorted order, contributing zero drops.
    \end{itemize}
    
    Consequently, drops only occur at two structural boundaries:
    \begin{enumerate}
        \item The old-new boundary: The transition from the end of the old section to the start of the new section contains at most one drop. This drop is strictly bounded by the total span of the current array: $\max(A) - \min(A) = OPT$.
        \item The internal sections boundaries: Within each block $B_i$, a single drop may occur at the boundary between $T_i$ and $O_i$. The magnitude of this internal drop is bounded by the span of that specific block: $\max(B_i) - \min(B_i)$.
    \end{enumerate}
    
    Because the blocks are globally monotonic (\cref{cl:global-monotonicity}), their spans are strictly disjoint. The sum of the spans of all disjoint blocks telescopes and cannot exceed the total span of the current elements:
    \[ \sum_{i=1}^{\sqrt{n}} \left( \max(B_i) - \min(B_i) \right) \leq \max(A) - \min(A) = OPT \]
    
    Summing these components, all drops across the structure is bounded by $2 \cdot OPT$. 
    Substituting this into our total variation bound yields:
    \[ ALG \le 2(2 \cdot OPT) + OPT = 5 \cdot OPT \]
    Since $ALG \le 5 \cdot OPT$, the algorithm maintains an $O(1)$ competitive ratio at all times.
\end{proof}

==> DST_operations.tex <==
We now describe the internal subroutines used by the \dst operations.


\begin{itemize}

\item \textbf{\addmax($i,y$):}
Given an $i$-level \dst\ whose last position is a hole, and an element $y$
that is larger than every element currently stored in the \dst, this
operation places $y$ in the hole.

\item \textbf{\swaphole($D,D'$):}
Suppose $D$ and $D'$ are two adjacent \dsts, possibly of different levels, with a hole at their common boundary that currently belongs to $D$. This operation transfers ownership of the hole from $D$ to $D'$.

\item \textbf{\movehole($i$):}
Given an $i$-level \dst\ with a hole at the end of a section of some non-last level-$(i-1)$ block $B_j$, this operation moves the hole to the first position of the last level-$(i-1)$ block. The section containing the hole is the original section if $B_j$ is a first block, and either the transfer section, or the original section when the transfer section is empty, if $B_j$ is a middle block.

\item \textbf{\slide($i$):}
Suppose we are given an $i$-level \dst\ with a hole at the beginning of the \dst. This operation moves the hole to the right of (and outside) the \dst.

\item \textbf{\routehole($i$):} Suppose in an $i$-level \dst, there is a hole that appears in an arbitrary position. This operation moves this hole to the right of (and outside) the $i$-level \dst, while compacting the remaining elements in the \dst.

\end{itemize}

In addition to the operations above, we also have two operations that are used for re-sizing the recursive structure of the \dst. These operations are described below and the next subsection describes the conditions that invoke these operations.

\begin{itemize}

\item \textbf{\mergeblock($i$):} This operation is applied on the $i$-level \dsts that constitute the level-$i$ sections of a level-$i$ first or middle block. The algorithm re-sorts all the elements in the block and creates a single $i$-level \dst, which is designated as the only (original) section of the block.

\item \textbf{\splitblock($i$):} This operation is applied on the $i$-level \dst that constitutes the only (original) section of a level-$i$ last block, or on 
any of the sections that constitute a level-$i$ first block.
The algorithm re-sorts all the elements in the block and creates two $i$-level \dsts of equal size, which respectively become the only (original) section of two level-$i$ blocks.


\end{itemize}

See \cref{fig:dst-call-structure} for the call relation between the operations.

\input{figures/DST_operations_relations}



















  




==> New_DST_files/DST_cost.tex <==
\begin{lemma}
\label{cl:dst-cost}
Let $S$ be an $i$-level \dst. Then, for every
threshold $z$,
\[
    cross_z(S)\le 4i.
\]
Consequently, if all elements of $S$ lie in an
interval $I$, then
\[
    cost(S)\le 4i|I|.
\]
\end{lemma}


==> New_DST_files/DST_delete.tex <==
% To delete an element $x$ from an $i$-level \dst,
% we remove $x$ from its cell, leaving a hole.
% We then invoke \routehole($i$), which moves the
% hole to the last position of the \dst.

%Finally, we release this last cell from the \dst\ and apply \rebuild\ to restore any resulting structural violations.


\begin{claim}
\label{cl:delete-invariants}
The \delete\ operation maintains all structural
invariants of the \dst, while creating a hole
in its last position.
\end{claim}

We now bound the recourse of the \delete operation. 
Excluding rebuilds, the recourse is bounded by \Cref{cl:route-hole-recourse}.
So, we focus on bounding the recourse due to rebuilds.
Although a single \rebuild may move
many elements, we show that its recourse can be amortized
to previous element deletions, losing only a factor of $O(d)$.
Recall that \rebuild is called only by \swaphole, 
if a Block Size invariant is violated. So, the first 
step is to bound the recourse due to \rebuild 
against the number of \swaphole operations. 

The next claim applies to the \dst at the highest level
$d$ that is not contained inside any other \dst. We also
assume, w.l.o.g., that initially the $d$-level \dst is a 
sorted array.

We are now ready to prove the overall recourse bound.
Note that this now includes recourse due to rebuilding.
As in the previous, we assume that the $d$-level \dst
is not contained any other \dst, and that it is initially
a sorted array.

\begin{lemma}
\label{cl:delete-total-recourse}
A prefix of $k$
\delete\ operations on a $d$-level \dst\ incurs
$O(k d^4)$ recourse in total. 
\end{lemma}

\begin{proof}
By \Cref{cl:route-hole-recourse}, each deletion
incurs $O(d^3)$ recourse excluding rebuilding.
Moreover, we note that in all operations, 
\swaphole is always preceded by an \addmax,
which incurs $1$ unit of recourse. Therefore,
by \Cref{cl:delete-total-recourse}, the 
total recourse due to calls to \rebuild operations
is at most $O(d)$ times the total recourse due
to \addmax, which in turn, is bounded by 
\Cref{cl:route-hole-recourse}.
The lemma follows.
\end{proof}



==> New_DST_files/DST_interface.tex <==
%The interface of the \dst provides the following two operations: \textbf{\delete} and  \textbf{\slide}. 

The \dst\ interface supports the following two operations: \textbf{\delete} and \textbf{\slide}.

\begin{itemize}
    \item \textbf{\delete}: Given an element $x$ stored in the \dst, this operation deletes $x$ from the structure. The deletion creates a hole at the position of $x$, which is then routed to the end of the \dst while restoring all structural invariants. Thus, if the \dst initially contains the set of elements $S$, then after \delete$(x)$ it is a valid \dst containing exactly $S\setminus\{x\}$.
    
   % \item \textbf{\slide}:
    %The operation is applied to the underlying \dst after a hole is created at its beginning. It moves this hole from the leftmost recursive chain to the right end of the \dst. Thus, the empty position created at the beginning of the \dst is shifted through the structure and becomes an empty position at the end of the \dst.
\end{itemize}

==> New_DST_files/DST_interface_implementation.tex <==
%\sbalert{We need some nice connectors here... why do we need interface}

%The interface of the \dst provides the following two operations: \textbf{\delete} and  \textbf{\slide}. 

We now describe the implementation of the \delete\ and \slide\ operations.
\subsubsection{Implementation of \delete}


To execute \delete$(x)$, we remove $x$, creating a hole, and apply \routehole to move the hole to the end of the \dst. We then remove the final empty slot from the \dst.

\begin{claim}
\label{cl:delete-invariants}
The \delete\ operation preserves all structural invariants.
\end{claim}

\begin{proof}
Removing an element $x$ creates a hole while leaving all structural invariants otherwise unchanged. By \Cref{cl:route-hole-invariants}, \routehole$(i)$ routes the hole to the end of the \dst\ while restoring all structural invariants. Finally, removing the empty slot at the end only shrinks the interval occupied by the \dst\ and does not change the position or relative order of any element. Therefore, all structural invariants are preserved.
\end{proof}





%After the hole has been initialized, \slide routes this hole to the end of the
%underlying \dst. This is done using the hole-routing operations described
%above. By Claim~\ref{cl:route-hole-invariants}, routing the hole preserves all
%section-order invariants. When the hole reaches the end of the \dst, the final
%empty slot is removed. Removing this empty slot cannot violate any ordering
%invariant, since it removes no element.




%It remains only to restore the block-size invariants. During \slide, the only
%blocks whose sizes may increase are the leftmost blocks on the recursive chain:
%these are precisely the blocks that are extended by the initial step of
%\slide, which creates the hole at the beginning of the \dst. All other blocks
%that the hole passes through maintain their size, since the operation only
%exchanges the hole with an element of the block; the hole moves forward, but
%the number of occupied positions in the block remains unchanged.

%The only exception is the last block. When the hole reaches the end of the
%\dst, the final empty slot is removed, and therefore the last block may lose
%one position. This cannot create an overflow violation; it can only make the
%last block smaller, which is allowed for the last block.

%Thus, the only remaining possible size violations are overflows of the leftmost
%blocks extended at the beginning of \slide. For every such block whose size
%exceeds its allowed bound, we apply \splitblock. By
%Claim~\ref{cl: split-invariants-and-recourse}, each such split preserves all
%invariants. Therefore, after all necessary splits are performed, all invariants
%of the \dst are restored.



%\end{proof}



%\end{proof}




\begin{claim}
\label{cl:split-merge-recourse}
For a $d$-level \dst, during one execution of either \delete\ or \slide,
the amortized recourse caused by \splitblock\ and \mergeblock\ is
\[
O(d\cdot n^{1/d}\cdot 2^d).
\]
\end{claim}

\begin{proof}
Consider one boundary-size change at level $i$. A level-$i$
\splitblock or \mergeblock operation incurs $O(n^{i/d})$ recourse.
After either operation, the affected boundary block has size
$n^{i/d}$, and hence $\Omega(n^{i/d})$ further boundary-size changes
are required before another split or merge can occur on that boundary.
Thus, the amortized resizing cost is $O(1)$ per boundary-size change
at each level.

A call to \swaphole changes one boundary position in each of its two
\dsts, and therefore causes $O(d)$ such changes over their recursive
boundary chains. Hence, its amortized split/merge cost is $O(d)$.

By the analyses of \routehole and \slide, one execution of either
\delete\ or \slide makes
$O(n^{1/d}\cdot 2^d)$ calls to \swaphole. Therefore, these calls incur
\(
O(d\cdot n^{1/d}\cdot 2^d)
\)
amortized recourse from \splitblock and \mergeblock.

Finally, \delete removes the final empty position after \routehole
terminates. This creates at most one additional boundary-size change at
each level, contributing only $O(d)$ additional amortized recourse, which
is dominated by the bound above.
\end{proof}


\begin{claim}
\label{cl:delete-slide-recourse}
For a $d$-level \dst, each of the \delete\ and \slide\ operations incurs
\(
O(d\cdot n^{1/d}\cdot 2^d)
\)
amortized recourse.
\end{claim}

\begin{proof}
Excluding the recourse of \splitblock\ and \mergeblock, \delete\ incurs
$O(n^{1/d}\cdot 2^d)$ recourse by \Cref{cl:delete-recourse}, while
\slide\ incurs $O(n^{1/d}\cdot 2^d)$ recourse by
\Cref{cl:slide-recourse}.

By \Cref{cl:split-merge-recourse}, the amortized recourse caused by
\splitblock\ and \mergeblock\ during either operation is
\(
O(d\cdot n^{1/d}\cdot 2^d).
\)
Combining the two bounds gives
\(
O(d\cdot n^{1/d}\cdot 2^d)
\)
amortized recourse for each operation.
\end{proof}

==> New_DST_files/DST_invariants.tex <==
The following structural invariants are maintained throughout the update
operations performed on the \dst. We assume that all elements have distinct
values, which is w.l.o.g. by adding an infinitesimal perturbation to every
element.

For two sets of elements $A$ and $B$, we write $A<B$ if every element of
$A$ is smaller than every element of $B$. Comparisons involving an empty
set are interpreted as vacuous.

\begin{enumerate}
    \item \textbf{Number and Structure of Blocks.}
    Every level-$i$ section consists of either one block or exactly three
    blocks.

    If it consists of one block, this block is a last block and contains only
    an original section.

    If it consists of three blocks, they are, from left to right, a first
    block, a middle block, and a last block. The first and last blocks
    contain only original sections, while the middle block consists of a
    transfer section followed by an original section.

    Thus, a three-block section has the form
        $O_1 \mid T_2 \mid O_2 \mid O_3$.

    
    \item \textbf{Base-Level Sorting.}
    Every level-$1$ section is sorted in increasing order from left
    to right.
    
    
    \item \textbf{Block Sizes.}
    A section consists of either one block or three blocks,
    with the following size bounds:
    
    \begin{itemize}
        \item If the section consists of a single level-$i$
        block, its size is at most $12\cdot 2^i$.
    
        \item If the section consists of three level-$i$
        blocks, the middle block has size exactly $2^i$,
        the first block has size in
        \(
            [2^i,12\cdot 2^i),
        \)
        and the third block has size in
        \(
            [7\cdot 2^i,12\cdot 2^i).
        \)
    \end{itemize}
    
    These bounds guarantee that whenever a section has three
    blocks, the original section of its third block also has
    three blocks, unless it is at level $1$.
%    
    Indeed, a third level-$i$ block contains at least
    $7\cdot 2^i$ elements,
    if represented by a single block, could contain at most
    \[
        12\cdot 2^{i-1}=6\cdot 2^i<7\cdot 2^i.
    \]
    Therefore, it cannot consist of
    a single block.




    \item \textbf{Block Ordering.}
    Consider a level-$i$ section consisting of three blocks
        $O_1\mid T_2\mid O_2\mid O_3$.
    We require
    $O_1<O_2<T_2$
    and
        $O_2<O_3$.
    
    By the block sizes invariant above, $O_3$ must itself
    consist of three blocks, unless it is at the base level where we require
       $T_2<O_3$.
    Otherwise, we write $O_3$ as
        $O'_1\mid T'_2\mid O'_2\mid O'_3$.
    We require the following ordering on the sections:
        $O'_1<T_2<O'_2$.
    This also implies that
        $O'_1<T_2< T'_2\cup O'_2\cup O'_3$.

\end{enumerate}

A useful property of these invariants is that they ensure the 
minimum element in a \dst occupies the first cell of the array.The invariants also ensure the  that the maximum element occupies the last cell of the array:

\begin{claim}
\label{cl:new-dst-minimum}
In every nonempty $i$-level \dst, the minimum element is in the
leftmost cell.
\end{claim}


\begin{claim}
\label{cl:new-dst-maximum}
In every nonempty $i$-level \dst, the maximum element
is in the rightmost cell.
\end{claim}


==> New_DST_files/moving-overview.tex <==
We now describe how holes are moved through the recursive
structure of a \dst. We use five operations:
\downhole, \simpleslide, \slide, \routehole, and
\delete. Their implementations are given in the
following subsections.
Consider a three-block section
\[
    S=O_1\mid T_2\mid O_2\mid O_3.
\]
\begin{itemize}

    \item \downhole:
    This operation moves a hole from the end of $T_2$
    to the end of $S$. The difficulty is that
    $\min O_3$ may be smaller than the elements of
    $T_2$, so we cannot necessarily use it to fill
    the hole.

    Instead, the recursive structure of $O_3$
    allows us to use an element from its middle
    original section $O'_2$ to fill the hole.
    We then transfer the resulting hole into
    $T'_2$ using \swaphole\ and continue recursively.
    This requires only a constant number of element
    movements at each level.
    
    \item \simpleslide: To move a hole from the beginning to the end of $S$,
    we first move it through $O_1$ and fill it with
    $\min O_2$. The resulting hole is at the beginning
    of $O_2$. Since $T_2$ and $O_2$ form a single
    middle block, \swaphole\ moves the hole to the
    end of $T_2$ without moving any stored elements.
    Finally, \downhole\ moves it through the last
    original section $O_3$ to the end of $S$.
    This is the basic \simpleslide\ operation.

   
    \item \slide: The general \slide\ must also handle the case where
    $S$ is the last original section of a
    three-block section with a nonempty transfer $U$.
    In this case, the ordering $O_1<U<O_2$ prevents
    us from moving $\min O_2$ directly into $O_1$.
    Instead, we first move $\min U$ into $O_1$,
    move the resulting hole through $U$ using
    \simpleslide, and then move $\min O_2$ into $U$.
    The remaining steps are identical to \simpleslide.


    \Cref{fig:slide-zigzag} illustrates how these recursive
    calls unfold across levels, and in particular why the
    recourse of \slide$(i)$ is quadratic rather than linear.

    \input{new_figures/dst_recursive_movement}

    \item \routehole: The operation \routehole\ handles a hole at an arbitrary
    position, as created by a deletion. We first recursively
    move the hole to the end of its current section.
    If the hole is in $O_1$ or $T_2$, the remaining
    steps of \slide or \downhole, respectively,
    complete the operation. A hole in $O_3$ is already
    at the end of $S$.
    %
    The remaining case is a hole in $O_2$.
    We fill it with $\min O_3$ using \addmax,
    and then apply \slide\ to $O_3$.
    When $T_2$ is nonempty, the exceptional case
    of \slide\ performs the necessary rotation
    through $T_2$, preserving the ordering invariants
    while moving the hole to the end of the \dst.

    \item  \delete:  will simply remove the requested element,
    apply \routehole\ to move the resulting hole to
    the end of its \dst.
\end{itemize}

==> augmented_dynamic_sorting_trees.tex <==
\subsection{Augmented Dynamic Sorting Trees (\adst)}

%\dpalert{Write something.}\sbalert{Will add!}
%\sbalert{Do we need to expand this more?}
The Dynamic Sorting Tree (\dst) of the previous section maintains an array in
approximately sorted order under deletions alone. However, to solve our original problem, we must also support insertions. The Augmented Dynamic Sorting Tree (\adst) is the structure that achieves this. It maintains an array
of size $n$ in approximately sorted order under an arbitrary online
sequence of both insertions and deletions, while keeping the amortized
recourse small.
The key idea is to organize the \adst\ as a sequence of \dsts\ of geometrically decreasing levels, with the base level consisting of a sorted array.
%The key idea is to build the \adst\ as a sequence of \dsts of geometrically decreasing levels, terminating in a $1$-level \adst, which is simply a sorted array. 
To insert an element, we place it into an empty slot. To delete an element, we remove it from the \dst\ containing it, which creates a hole. The hole is then propagated to the end using the \moveany operation (see \Cref{subsec:moveany-implementation} for definition). Finally, after sufficiently many deletions, the \resort\ operation rebuilds the affected \adst\ from its current elements, ensuring that the \adst\ again has the required maximum size and resetting the deletion counter.


%To insert an element, we place it in an empty slot. To delete an element,
%we remove it from the DST that contains it. This leaves a hole, which we
%push to the end using the \slide\ and \moveany\ operations. Each level
%is rebuilt from time to time by a \resort\ operation to stay compact.



\subsubsection{The Structure of a $d$-Level \adst}\input{ADST_files/ADST_description}

%Description of a $d$-Level \adst}\input{ADST_files/ADST_description}

\subsection{Cost Bound for an \adst}\input{ADST_files/ADST_cost}

\subsection{Size bound for an \adst}\input{ADST_files/ADST_size}

\subsection{\adst: The Auxiliary Operations}\input{ADST_files/ADST_auxilary}

\subsection{\adst: The interface}\input{ADST_files/ADST_interface}


==> dynamic_sorting_trees.tex <==
We begin by introducing the {\em dynamic sorting tree} (\dst) data structure, which is a virtual data structure whose goal is to maintain the array in approximately sorted order {\em under deletions only}, while moving the holes created by deletion to the end of the array. We will later use the \dst data structure to construct an augmented dynamic sorting tree (\adst) data structure that will also support element insertions. Since an \adst will comprise a sequence of \dsts, we have to support an additional operation on \dsts to cascade an element deletion across the different \dsts comprising an \adst; we call this a {\em slide} operation. This operation moves a hole from the left of a \dst data structure to the right of the data structure, while keeping the \dst compact. 

\subsection{Description of a $d$-Level \dst}\input{DST_files/DST_description}

\subsection{Structural Invariants of a \dst}\input{DST_files/DST_invariants}

\subsection{Cost Bound for a \dst} \input{DST_files/DST_cost}

\subsection{The interface of the \dst} \input{DST_files/DST_interface}

\subsection{Basic Operations of a \dst}\input{DST_files/DST_operations}

\subsection{Re-sizing Operations of a \dst}\input{DST_files/DST_resizing}

\subsection{The \mergeblock($i$) Operation}\label{subsec:merge}\input{DST_files/DST_merge}

\subsection{The \splitblock($i$) Operation}\label{subsec: split}\input{DST_files/DST_split}

\subsection{The \addmax($i, y$) Operation} \input{DST_files/DST_add_max}

\subsection{The \swaphole Operation} \input{DST_files/DST_swap_hole}

\subsection{The \movehole($i$) Operation}\input{DST_files/DST_movehole}

\subsection{The \slide($i$) Operation}
\input{DST_files/DST_slide}

\subsection{The \routehole operation}\input{DST_files/DST_routehole}

\subsection{Implementation of the \dst Interface}\input{DST_files/DST_interface_implementation}



==> fully-dynamic-highcost.tex <==
    In this section, we consider a model where the adversary is also allowed to delete elements.
    We show an algorithm which uses $O(\log n)$ amortized recourse
    and achieves cost $O(\sqrt{n})$ with deletions.

    Note: This algorithm is based on the $O(\sqrt{n})$ cost algorithm with $m=n$ and no recourse found in~\cite{AABK23} (Section $4.1$).

    During the course of the algorithm, we let $t$ denote the
    current time step (the current number of insertions and deletions).
    For each level $i$ and time $t$, we let $n_i^{(t)}$
    denote the size of the virtual array at level $i$ at time $t$.
    We also let $t_i$ denote the last time step at which level $i$ was rebuilt
    (either because $i$ was created as the bottom level of recursion, or some level above $i$ was rebuilt).

    Our algorithm follows a similar framework as previous algorithms.
    When a new level $i$ is created as the bottom level of recursion during time $t_i$,
    we create $2\sqrt{n_i^{(t_i)}}$ blocks of size $\sqrt{n_i^{(t_i)}}/2$,
    each corresponding to a range of $1/\sqrt{n_i^{(t_i)}}$.
    We use the same procedure as before to place new elements into blocks
    and create a new level of recursion when there are no more overflow blocks available.
    For each deletion, we propagate the deletion down to the bottom level by
    filling the newly created hole at each level with the rightmost element
    of the corresponding block.
    Note that this preserves the property that each block only contains elements from a certain range,
    and that the filled cells in a block are always contiguous.
    At some time $t$ and for some level $i$, we rebuild level $i$ (and all subsequent levels)
    if either of the following conditions are met.
    \begin{enumerate}
        \item level $i$ is the bottom level and $n_i^{(t)} > \frac{4}{3} n_i^{(t_i)}$, i.e.,
        the current size of the virtual array at level $i$ exceeds $4/3$ times the initial size of the virtual
        array when level $i$ was last rebuilt.
        \item $n_{i+1}^{(t)} > \frac{7}{8} n_i^{(t)}$, i.e., the current size of
        level $i+1$ exceeds $7/8$ times the current size of level $i$.
    \end{enumerate}
    Thus we maintain the invariants that $n_i^{(t)} \le \frac{4}{3} n_i^{(t_i)}$ for the bottom level,
    and $n_{i+1}^{(t)} \le \frac{7}{8} n_i^{(t)}$ for all levels.

    We first claim that when we recurse and create a new level $i+1$,
    we have that $n_{i+1}^{(t)} \le \frac{5}{8} n_{i}^{(t)}$, i.e.,
    the size of the new level $i+1$ is at most $5/8$ times the current size of level $i$.
    This is because when we recurse, at least half of the original cells at level $i$ must be filled, so we have
    \[n_{i+1}^{(t)} \le n_{i}^{(t)} - \frac{n_{i}^{(t_i)}}{2} \le n_{i}^{(t)} - \frac{3}{8}n_{i}^{(t)}
    = \frac{5}{8}n_{i}^{(t)}.\]

    \subsection{Recourse}
    We first show that we use $O(\log n)$ recourse.
    Clearly, propagating the deletions uses at most $O(\log n)$ recourse per deletion.
    To analyze the recourse used in rebuilding levels, imagine that
    each deletion adds $4$ tokens to each current level.
    Since the depth of the tree is $O(\log n)$, this creates $O(\log n)$ tokens per deletion as desired.
    We now show these tokens are enough to pay for the rebuilds.

    For the first type of rebuild, when $n_i^{(t)} > \frac{4}{3} n_i^{(t_i)}$,
    note that we must have received at least $n_i^{(t_i)}/3$ deletions since the last rebuild of level $i$.
    This corresponds to $\frac{4}{3} n_i^{(t_i)}$ tokens, which is exactly enough
    to pay for the $n_i^{(t)}$ recourse steps needed to build level $i$.
    (Note that we actually have enough budget to pay for this type of rebuild at all levels instead
    of just the bottom level, but just doing this rebuild at the bottom level is sufficient for the algorithm to work.)

    For the second type of rebuild, when $n_{i+1}^{(t)} > \frac{7}{8} n_i^{(t)}$,
    recall that we have $n_{i+1}^{(t_{i+1})} \le \frac{5}{8} n_{i}^{(t_{i+1})} \le \frac{5}{8} n_{i}^{(t)}$.
    Thus
    \[n_{i+1}^{(t)} - n_{i+1}^{(t_{i+1})} \ge \frac{7}{8} n_i^{(t)} - \frac{5}{8} n_{i}^{(t)}
    = \frac{1}{4} n_{i}^{(t)},\]
    implying that we must have received at least $\frac{1}{4} n_{i}^{(t)}$ deletions
    since the last rebuild at level $i$.
    This corresponds to $n_{i}^{(t)}$ tokens, which is exactly enough to rebuild level $i$.

    \subsection{Cost}
    We now analyze the cost at any time in the execution of the algorithm.
    At any level $i$, the cost is asymptotically bounded by
    the number of blocks (which each incur a cost of $O(1)$ from the boundaries of the block)
    plus the number of filled cells times the range of a block (the total cost within blocks).
    Thus the total cost at level $i$ is at most
    \[O\left(\sqrt{n_{i}^{(t_i)}} + n_i^{(t)} \frac{1}{\sqrt{n_i^{(t_i)}}}\right).\]
    Since $n_i^{(t_i)} \le n_i^{(t)} \le \frac{4}{3} n_i^{(t_i)}$, the cost is $O\left(\sqrt{n_i^{(t)}}\right)$.
    We have at all times that $n_{i+1}^{(t)} \le \frac{7}{8} n_i^{(t)}$,
    so the total cost at any time is at most
    \[\sum_{i} \sqrt{\left(\frac{7}{8}\right)^i n} = O(\sqrt{n}).\]


    %    \begin{theorem}
    %        \label{thm:main}
    %        For any $c \in \NN_{\ge 2}$, there is an $O(nc)$ algorithm for online sorting which uses
    %        an amortized budget of $2^c$ each iteration and achieves a cost of $O(2^c n^{1/c})$.
    %    \end{theorem}
    %    Setting $c$ to any constant, we have the following corollary:
    %    \begin{corollary}
    %        For any constant $c \ge 2$, there is an algorithm for online sorting
    %        which uses an amortized budget of $O(1)$ each iteration and achieves a cost of $O(n^{1/c})$.
    %    \end{corollary}
    %    By setting $c = \log(\log (n))$, we have the following corollary:
    %    \begin{corollary}
    %        There is an algorithm for online sorting which uses
    %        an amortized budget of $O(\log n)$ each iteration and achieves a cost of $O(n^{1/\log(\log(n))})$.
    %    \end{corollary}
    %
    %    \begin{proof}{\ref{thm:main}}
    %        We inductively define a sequence of algorithms $f_2$, \dots, $f_c$, where each algorithm $f_i$
    %        uses an amortized budget of $2^{i-1} - 2$ and incurs a cost of $O(2^i n^{1/i})$.
    %        The base case of $i=2$ is achieved by the classical algorithm without recourse.
    %
    %        For $i \ge 3$, assume there is an algorithm $f_{i-1}$ which satisfies the conditions above.
    %        We follow the idea of the classical recursive algorithm, but split the $n$ cells into $2n^{1/i}$ blocks,
    %        each containing $(n^{1 - 1/i})/2$ cells which cover a range of $n^{-1/i}$ possible elements.
    %        We use the same procedure as before to decide which block to place each new element into.
    %        Then within each block, we use algorithm $f_{i-1}$ to determine where in the block to place
    %        each new element.
    %        When we run out of blocks to place a new element, we first use recourse steps within each block
    %        to shift all of the elements to the leftmost cells of that block.
    %        We then recurse as before on the remaining empty cells.
    %    \end{proof}


%\newpage


% \subsection{$O(1)$ cost O($n^{1/3}$) recourse}
% First, we assume that after any deletion, an insertion follows; otherwise, we ignore the deletion operation, as it does not increase the cost.
% We also assume that, at the beginning of the algorithm's run, the array is sorted. \ov{Need to see how we can smooth this assumption out later on.}

% Now, the algorithm maintains two separate parts of the array, which are one after the other.
% One for the elements before the last time the array was completely sorted, and another for the elements inserted after the last time the array was sorted. 
% We will refer to the first part as old and the second as new, in the same manner, we will refer to the elements in them as old and new elements accordingly.

% For the separation to be maintained, any time an element $x$ is inserted in position $i$ in the section of the old elements we swap it with the last element in the array that is old and $x$ is added to the new section, where its position will later be determined by an algorithm for insertion only for the new elements in the array.
% Note that this separation only has a cost of at most $1$ and requires recourse of at most $O(1)$.
% First, we always sort the array for every $n^{2/3}$ operations, which brings us to the initial configuration of a sorted array.

% \subsubsection{The data structure for old elements}
% We separate the original array into blocks of size $n^{2/3}$.
% Each block will also be separated into sub-blocks of size $n^{1/3}$.
% For any sub-block other than the first, we will have two parts that change in size during the run of the algorithm.
% At the start of each such sub-block, we will have elements from the next sub-block in a section that will be referred to as the transferred section.
% Immediately following it in the block, we will have elements from the original sub-block, which will be referred to as the origin section.
% The first sub-block of each block will be maintained in a different way.
% It will have three different sections.
% The first one will be elements from the next block, which will be refered to as block-tranferred and they will comprise of the elements that will be transferred to block $i$ from block $i+1$.
% This section will considered entirely distinct from the sub-block and will be handled separately.
% The second one will also be the transferred section as before.
% The third one will still be the origin section.

% Our structure will maintain the following invariants for sub-blocks in a given block $j$:
% \begin{itemize}
%     \item For a sub-block $i > 1$, the values of elements in sub-block $i$ are always smaller than the values of elements in block $i+1$.
%     \item For the first sub-block, the values of the elements in the block in the origin and transferred section will be smaller than the values of elements in sub-block $2$ of the same block, and as a result, for all other sub-blocks as well.
%     \item For a sub-block $i > 1$, both the transferred and the origin section of each block will be completely sorted.
%     \item For the first sub-block, the origin section will be completely sorted, and the transferred section will comprise two sorted arrays.
%     \item The elements in the transferred section of any sub-block $i$ came from the origin section of sub-block $i+1$.
% \end{itemize}

% Our structure will maintain the following invariants for blocks:
% \begin{itemize}
%     \item For any block $i$, the values of elements in block $i$ are always smaller than the values of elements in block $i+1$.
%     \item The elements in the transferred section of any block $i$ came from the origin section of block $i+1$.
% \end{itemize}

% Note that at the beginning (when the array is completely sorted), all invariants are maintained.
% The algorithm is now going to be defined as follows:
% First, after any $n^{1/3}$ deletion operations in a block $j$, we will completely sort the elements in the block.
% Let $j$ be the index of the block an element was removed from, and let $i$ be the index of the sub-block it was removed from. Let $x$ be the last element in the new section that was moved into the block.
% We start by describing the algorithm for the case where $i>1$.
% In sub-block $i$, we shift the elements in the sub-block such that $x$ is located after the last element in the transferred section of sub-block $i$.
% Now, $x$ is swapped with the first element in the origin section of sub-block $i+1$.
% Using \cref{cl:origin-never-empties}, such an element $y_{i+1}$ must exist.
% Now, for $k$ starting from sub-block $i+1$ up to sub-block $n^{1/3}$, we swap the location of $x$ with the first element in the origin section of sub-block $k$, $y_{k+1}$, using the same notations.
% The operation for the final block, i.e. block $n^{1/3}$, is slightly different.
% We take the smallest element $z$ in block $j+1$ and swap it with $x$. Note that $z$ must be in the first sub-block (which contains the smallest elements) of block $j+1$.

% Now, if $i$ is the first sub-block we split into cases:
% \begin{itemize}
%     \item If the element is deleted from either the transferred or origin section of the sub-block, the transferred section is completely sorted, and $x$ is moved such that it is in the end of the transferred section. The process in block $j$ continues as written above.
%     \item If the element is deleted in the transferred section of the block $j$, we run the algorithm recursively, such that $x$ is at the end of the transferred section, and continue the algorithm as will be described below. \ov{TODO: rewrite differently, the recursion should be explained more carefully}
% \end{itemize}

% The operation for the following blocks works as follows:
% For any $\ell$ from $j+1$ to $n^{1/3}$ we swap $x$ with the smallest element in the origin section of the first sub-block. Then, we swap $x$ with position of $x$ with the element $d$, which is the first element after the transferred section of the $\ell$ block. The process continues until the final block, the $n^{1/3}$ block. 
% \subsubsection{The data structure for new elements}
% The data structure used is the data structure for $O(1)$ cost and $O(\sqrt{n)}$ recourse.
% A deletion in this section is handled as written previously.
% A deletion in the old section creates a hole at the beginning of the data structure, which is then moved to the end using the same process.
% \ov{TODO: Go in to more details}



==> fully-dynamic-lowcost.tex <==

% Introduce the A-DST briefly, state the guarantees, and explain intuitively what it is trying to achieve... 

\subsection{From Deletions to Insertions: The \adst}

%Explain the basic idea using a DST followed by a small sorted array that receives newly inserted elements.

% Describe a deletion-insertion pair.
% Delete from the appropriate component, pass the hole to the
% end, and insert the new element into the sorted suffix.

% Explain why the suffix cannot keep growing. Introduce periodic rebuilding, then replace the sorted suffix by a lower-level \adst\ to obtain the recursive construction.

%Add fig. if possible.... or you can refer to later figs. which will come in the following subsections...

\subsection{The Structure of a $d$-Level \adst}

\paragraph{Recursive structure.}
% Define an i-level \adst\ as an i-level \dst\ followed by an (i-1)-level \adst.... explain the base case and the unrolled view.


\paragraph{Structural invariants.}
% Specify the component size bounds and the ownership of positions... define the rebuilding counters, thresholds, and what is reset when rebuilding occurs.

\paragraph{Size bound \& Sorting-cost bound}


\subsection{Operations and Implementation Details}

\paragraph{Interface.}
% State the insertion and deletion operations....
%this should be written in the same same spirit as the beginning of this section... but of course with more details...

\paragraph{Moving a hole through an \adst.}

\paragraph{The deletion operation.}

\paragraph{The insertion operation.}

\paragraph{Rebuilding.}

\subsection{Recourse Bound}

\paragraph{Recourse of hole movement.}

\paragraph{Amortized cost of rebuilding.}

\paragraph{Overall bound.}


%Also make figs. similar like the previous section... and whenever possible add. But we shouldn't overdo also... 

%Also if we feel

\input{augmented_dynamic_sorting_trees}

\subsection{Cost Bound}


We use a \(d\)-level \adst, where \(d=\sqrt{\log n}\). Let \(I\) be the
interval spanned by the input elements. By \Cref{cl:adst-cost}, the cost
of the maintained structure is
    $cost(A)=O(d^2)\cdot |I|.$
Since \(d=\sqrt{\log n}\), this becomes
    $cost(A)=O(\log n)\,|I|.$
Since \(OPT=|I|\), the competitive ratio is
\(
    O(\log n).
\)

\subsection{Recourse Bound}

We again use a \(d\)-level \adst with \(d=\sqrt{\log n}\). By
\Cref{cl:adst-delete-recourse}, the amortized recourse of a deletion in a
\(d\)-level \adst is
$O(d\cdot n^{1/d}\cdot 3^d)$.

An insertion is performed recursively in the auxiliary part of the \adst until
it reaches a level-\(1\) sorted array. By the size invariant of the \adst, this
array has size at most \(n^{1/d}\), and therefore the recourse of an insertion
is $O(n^{1/d})$.
Thus, deletions dominate insertions, and the amortized recourse per update is
$O(d\cdot n^{1/d}\cdot 3^d)$.
Since \(d=\sqrt{\log n}\), we have
   $ n^{1/d}=2^{O(\sqrt{\log n})}$ and 
   $3^d=2^{O(\sqrt{\log n})}.$
Therefore,
$ d\cdot n^{1/d}\cdot 3^d =
    2^{O(\sqrt{\log n})}.$
Hence the amortized recourse per update is
    $2^{O(\sqrt{\log n})}.$






==> lower-bound-overview.tex <==
\subsection{Proof Overview.}

\paragraph{The value hierarchy}

Fix integers \(B,d\), and let \(N=B^d\).  Initially there are \(N\)
distinct \emph{ordinary values}
\[
    x_j=\frac{j-\tfrac12}{2N},
    \qquad j=1,\ldots,N,
\]
together with two permanent values \(0\) and \(1\).
These two permanent values are never replaced.  Since every instance
contains both \(0\) and \(1\), every solution has cost at least \(1\);
placing all values in increasing order has cost exactly \(1\).
Hence \(OPT=1\), and a \(C\)-competitive algorithm always has cost at
most \(C\).

We organize the \(N\) ordinary values in a fixed \(B\)-ary hierarchy of depth $d$.
The permanent values \(0\) and \(1\) are not part of this hierarchy.
The root corresponds to the value interval \([0,1/2]\) and contains all
\(N\) ordinary values.  Every internal interval is divided into \(B\)
equal consecutive subintervals, which form its children.  Thus each
child contains a consecutive equal-size group of ordinary values, and
the hierarchy is a complete \(B\)-ary tree of depth \(d\).

We use the same notation \(I\) for a hierarchy node and for its
corresponding value interval.  Let \(N_I\) denote the number of ordinary
values contained in \(I\).  If \(I\) has depth \(k\), then
\[
    N_I=\frac{N}{B^k},
    \qquad
    |I|=\frac{1}{2B^k}
        =\frac{N_I}{2N}.
\]
In particular, every leaf contains exactly one ordinary value.

The hierarchy is purely an auxiliary structure in value space and has
no relation to the physical locations of the values in the algorithm's
array.  Values belonging to the same hierarchy interval may occupy
widely separated cells, while values belonging to different intervals
may be arbitrarily interleaved.  A value's membership in the hierarchy
is fixed throughout the construction.

The adversary uses the hierarchy to choose ordinary values iteratively.
Whenever it reaches a hierarchy interval for the first time, it
classifies the children of that interval into two roles, called
\emph{target} and \emph{buffer}.  This classification is chosen
adaptively from the current physical arrangement of the corresponding
values in the array.

\paragraph{The recursive adversary.}

The adversary works in rounds.  During the forward phase it repeatedly
descends the fixed \(B\)-ary hierarchy and replaces a live ordinary value
by a fresh copy of \(1\).  An ordinary value is \emph{live} if it is still
present in the array, i.e., it has not yet been replaced during the
current forward phase.  An interval \(I\) is \emph{entered} the first time
a descent reaches \(I\) in the current round.

When \(I\) is entered, all \(N_I\) ordinary values contained in \(I\)
are still live.  Indeed, replacing any value in \(I\) would already have
required an earlier descent through \(I\).  At this point the adversary
protects some of the children of \(I\) as \emph{buffers} and initially
allows recursion only through the remaining \emph{target} children.

We now describe how these labels are chosen.  The outer \(B/2\) children
of \(I\), in value order, are declared buffer children.  For the middle
\(B/2\) children, the adversary considers all ordinary values belonging
to these children in their current left-to-right order in the array and
divides this order into consecutive windows of \(8N_I/B\) values.

A labeling assigns each middle child of \(I\) either \emph{target} or
\emph{buffer}.  Accordingly, an ordinary value in \(I\) is called a
\emph{target value of \(I\)} or a \emph{buffer value of \(I\)} according
to the label of the child of \(I\) that contains it.  This classification
is with respect to \(I\): if a child \(J\) is later entered, its own children
receive a new target--buffer labeling (with respect to \(J\)) independently.
%MERGE
%Upon entering \(I\), each ordinary value in \(I\) is classified
%label of the child of \(I\) containing it.  This classification is only
%with respect to \(I\).  If a child \(J\) of \(I\) is later entered, then
%the children of \(J\) receive their own target--buffer classification,
%independently of the label that \(J\) received as a child of \(I\). The classification of a value is per interval. The classification of a value may be different for different intervals $I$ that contains this value.

Given a labeling, each window contains some values belonging to target
children and some belonging to buffer children.  We call a window
\emph{balanced} if it contains at least \(N_I/B\) values of each type.
The adversary chooses the labeling of the middle children that maximizes
the number of balanced windows.  A coloring argument shows that,
regardless of the current physical arrangement, some labeling gives
\(\Theta(B)\) balanced windows.  The chosen labels remain fixed for \(I\)
throughout the forward phase.

The balanced windows will later show that the adversary cannot replace
many target values while keeping most buffer values fixed without forcing
a large array cost.

For an entered interval \(I\), we say that a buffer value of \(I\) has
\emph{moved} once that ordinary value changes its array cell after \(I\)
was entered.  Replacing the value by a fresh copy of \(1\) is not
considered a move.  Fix a sufficiently small universal constant
\(\varepsilon>0\).  Every entered interval starts \emph{unpaid}.  While
fewer than \(\varepsilon N_I\) of its buffer values have moved, only its
target children are available for further descent.  Once
\(\varepsilon N_I\) buffer values have moved, \(I\) becomes \emph{paid},
and all of its children become available for the remainder of the forward
phase.  Thus an interval becomes paid only after \(\Omega(N_I)\) distinct
buffer values have moved.

At each step of the forward phase, the adversary starts at the root and
searches for a live ordinary value.  At an unpaid interval it may continue
only through target children, whereas at a paid interval it may continue
through any child.  Thus a buffer child of an unpaid interval is ignored
even if it still contains live ordinary values.

Whenever the search reaches a live leaf, the adversary replaces its
ordinary value by a fresh copy of \(1\), waits for the algorithm to
complete its response, and then starts the next search again from the
root.  The forward phase terminates when no live ordinary value can be
reached using the currently available children.  Live ordinary values
may still remain, but each such value is then hidden below a buffer child
of some unpaid interval.

Finally, the reverse phase deletes the copies of \(1\) inserted during
the forward phase and reinserts the ordinary values that were removed.
Thus the original multiset is restored, and the next round starts from
whatever physical arrangement the algorithm produced.

\paragraph{Cost through a value interval.}

To analyze an unpaid interval \(I\), we measure how much of the current
array cost passes through its value range.  For every consecutive pair of
values \(x,y\) in the array, we count the length of the portion of the
value interval between \(x\) and \(y\)(such that $x < y$) that lies inside \(I\), namely
\[
    \bigl|I\cap[x,y]\bigr|.
\]
The cost passing through \(I\) is the sum of these contributions over all
consecutive pairs in the array.

In particular, if along the array the values go from the middle half of
\(I\) to a value outside \(I\) and later return to the middle half, then
they contribute \(\Omega(|I|)\) cost passing through \(I\).  Moreover,
costs passing through disjoint value intervals sum to at most the total
array cost.

\paragraph{Local forcing at an unpaid node.}

Fix an entered interval \(I\) that is still unpaid.  The target--buffer
labeling gives \(\Theta(B)\) balanced windows in physical array order.
Order the balanced windows from left to right.  From the first chosen
window select \(N_I/B\) buffer identities, from the next select
\(N_I/B\) target identities, from the next select buffer identities
again, and continue in this way.  
This gives alternating groups of selected target and buffer identities
in physical array order.  Since all of these identities were chosen from
windows containing only identities from the middle children of \(I\),
every selected identity has value in the middle half of \(I\).

For each selected buffer group, if all of its \(N_I/B\) selected
identities have left the cells they occupied when \(I\) was entered, then
all of these identities have moved.  Otherwise, choose one selected
identity that still occupies its original cell and call it the
\emph{reference identity} of that buffer group.

Now consider one selected target group and its two neighboring buffer
groups.  If either neighboring buffer group has no reference identity,
then that buffer group already certifies \(N_I/B\) moved buffer
identities.  Otherwise, let the reference identities of the two
neighboring buffer groups be the left and right reference identities for
this target group.
Since the selected target group lies between the two buffer groups in
physical array order, every cell originally occupied by one of its
selected target identities lies between these two reference identities.

Importantly, the selected identities need not be consecutive in the
array.  We never treat them as if they were.  Instead, once the two
reference identities are fixed, we consider the actual sequence of
consecutive occupied values in the array between them, including all
intervening identities.

Suppose one of the selected target positions currently contains a value
\(y\notin I\).  Let \(x_L\) and \(x_R\) be the values of the two reference
identities.  Both lie in the middle half of \(I\).  Along the actual
array order from \(x_L\) to \(y\), the sum of the consecutive absolute
differences is at least \(|x_L-y|\), and similarly the cost from \(y\)
to \(x_R\) is at least \(|y-x_R|\).  Since \(y\notin I\) and
\(x_L,x_R\) lie in the middle half of \(I\), both distances are at least
\(|I|/4\).  Hence the portion of the array between the two reference
identities contributes at least \(|I|/2\) to the current array cost.

Suppose instead that none of the selected target positions contains a
value outside \(I\).  Then all \(N_I/B\) of these positions currently
contain values from \(I\).  Any such value belongs either to a target
identity that is still live or to a buffer identity that has moved into
one of these positions.

It remains to justify that these contributions can be summed over the
\(\Theta(B)\) selected target groups.  The selected target positions are
disjoint, so each identity occupying one of these positions is counted
there at most once.  A selected buffer group is adjacent to at most two
target groups.  Thus, even allowing for a moved buffer identity also to
occupy one selected target position, every buffer movement is counted
only a constant number of times.

The cost contributions can also be summed.  Whenever two target groups
use the same buffer group between them, they use the same reference
identity from that group.  Hence the corresponding portions of the array
may meet at this common identity, but contain no common consecutive pair
of occupied values.
Since the selected target groups contain
\(\Theta(B)\cdot N_I/B=\Theta(N_I)\) positions altogether, the preceding
accounting gives the following quantitative form of the local forcing
statement.  


For a fixed interval \(I\) we use the following definitions:
\begin{itemize}
\item Let \(U_I\) be the number of target identities of \(I\) that are
currently live.  
\item Let \(V_I(A)\) denote the current cost passing
through the value interval \(I\).
\end{itemize}
Then, we claim that for every \emph{entered} interval $I$ and, while \(I\) is  \emph{unpaid} we have
\[
U_I+\frac{2N}{B}V_I(A)
    \ge \gamma N_I
\]
for some constant \(\gamma>0\).

Thus for unpaid interval either \(\Omega(N_I)\) target identities remain live or
\(
    V_I(A)=\Omega(B|I|).
\)

\paragraph{Why the forward phase replaces most values.}

Let \(A\) denote the array when the forward phase terminates, and let
\(S\) be the set of ordinary values that are still live.  At the end of the forward phase, every surviving ordinary value lies
inside a buffer child of some entered unpaid interval.  We follow
the root-to-leaf path containing the value.  At a paid interval all
children are available, while at an unpaid interval every target child
is available.  Thus, as long as the child containing the surviving value
is available, that child must have been entered.  Since an entered leaf
cannot still contain a live ordinary value, at some point this path must
reach an unpaid interval whose buffer child contains the value.
let \(J\) be the first child that is a buffer child
of an unpaid interval \(I\).  Since \(J\) was never available, none of
the ordinary values in \(J\) were replaced.  Thus the surviving values
are contained in disjoint buffer subtrees of unpaid intervals, and our
goal is to bound the total population of these blocked subtrees.

For an unpaid interval \(I\), the term \(U_I\) in the local forcing
inequality is precisely the surviving mass that continues recursively
into the target children of \(I\).  We bound this term using the
recursive bounds for those children.  Substituting this bound into the
local forcing inequality then bounds the entire population \(N_I\), and
hence all survivors in \(I\), in terms of \(V_I(A)\).

For a paid interval there is no obstruction at the current level: all
of its children are available, and every child containing a surviving
value must have been entered.  We therefore recurse into all such
children.

The following recursive bound summarizes this bookkeeping.

\begin{lemma}[Survivor bound]
There is a universal constant \(\alpha>1\) such that, if \(I\) is an
entered interval of height \(h\), then at the end of the forward phase
the number \(S_I\) of live ordinary values in \(I\) satisfies
\[
    S_I
    \le
    \frac{2N}{B}\,\alpha^h V_I(A).
\]
\end{lemma}

\emph{Proof sketch.} The lemma follows by induction on the height.  At a paid interval one
simply applies the induction hypothesis to its entered children.  At an
unpaid interval, the local forcing inequality bounds \(N_I\), and hence
all possible survivors in \(I\), by the cost through \(I\) together
with the live target values; the latter are bounded recursively in the
entered target children.  Since the children of \(I\) are disjoint value intervals,
\[
    \sum_{J\text{ child of }I} V_J(A)\le V_I(A).
\]
Thus the inductive bounds for the relevant children can be summed and
expressed again in terms of \(V_I(A)\).  For a paid interval this
directly gives the desired bound.  For an unpaid interval, substituting
the resulting bound on \(U_I\) into
\[
    U_I+\frac{2N}{B}V_I(A)\ge \gamma N_I
\]
adds a constant factor. 

Applying the survivor bound to the root \(r\), which has height \(d\),
gives
\[
    |S|
    = S_r
    \le
    \frac{2N}{B}\alpha^d V_r(A)
    \le
    \frac{2N}{B}\alpha^d C.
\]
We choose
\begin{align}
    B \ge 8\alpha^d C \label{eq:choice-of-B}
\end{align}
and therefore
\[
    |S|\le \frac N4.
\]
Consequently, at least \(3N/4\) ordinary values are replaced during
every forward phase.

\paragraph{At least half the values lie in paid intervals at every level.}

We next show that, at every internal level of the hierarchy, the paid
intervals contain at least \(N/2\) ordinary values in total.  Fix such
a level, and let \(\mathcal U\) be the intervals at this level that are
not paid.  Every \(I\in\mathcal U\) leaves at least \(N_I/2\) values
live: if \(I\) was never entered then all its values survive, while if
\(I\) was entered but remains unpaid then all values in its buffer
children survive.  Since at most \(N/4\) ordinary values remain live,
\[
    \frac12\sum_{I\in\mathcal U}N_I\le \frac N4.
\]
Thus, at every internal level, the paid intervals contain at least
\(N/2\) ordinary values in total.

As an immediate consequence, summing over the \(d\) internal levels,
\[
    \sum_{I\text{ paid}} N_I \ge \frac{Nd}{2}
    = \Omega(Nd).
\]

\paragraph{From paid intervals to recourse.}

The key claim is that the movements paying different intervals can be
counted without overlap.  More precisely, for each paid interval \(I\),
take the \(\varepsilon N_I\) distinct buffer values whose movements make
\(I\) paid.  Across all paid intervals, these correspond to
\(\varepsilon\sum_I N_I\) distinct recourse events.

To see this, consider two paid intervals.  If they are incomparable,
their buffer values are disjoint.  Now suppose \(J\subsetneq I\).  If
\(J\) is entered before \(I\) is paid, then \(J\) lies inside a target
child of \(I\), so a buffer value of \(J\) cannot be a buffer value of
\(I\).  If \(J\) is entered after \(I\) is paid, then any movement used
to pay \(J\) occurs after \(J\) is entered, and hence after the movements
used to pay \(I\).  Thus, even if the same value is used at both levels,
it must move twice.

Therefore
\[
    \operatorname{recourse}
    \ge
    \varepsilon\sum_{I\text{ paid}} N_I
    =
    \Omega(Nd).
\]
Since a round contains only \(O(N)\) updates, its amortized recourse is
\begin{align}
    \frac{\Omega(Nd)}{O(N)}
    =
    \boxed{\Omega(d)}. \label{eq:recourse-is-d}
\end{align}


\paragraph{Choosing the parameters}
It remains to choose the branching factor \(B\) and the depth \(d\).
By \eqref{eq:choice-of-B}, we choose \(B\) to be the smallest power of two
satisfying the required number of surviving identities.  Hence
\[
    B=\Theta(\alpha^d C).
\]
The construction uses
\(
    N=B^d
\)
, or
equivalently
\(
    B^d\le N.
\)
Since \(\alpha\) is a constant and
\(B=\Theta(\alpha^d C)\),
\[
    \log B
    =
    \Theta\!\bigl(\log(C+1)+d\bigr).
\]
Thus the condition \(B^d\le N\) is satisfied whenever
\[
    d\bigl(\log(C+1)+d\bigr)=O(\log N).
\]
We may consequently choose
\[
    d=
    \Theta\!\left(
        \frac{\log N}
        {\log(C+1)+\sqrt{\log N}}
    \right),
\]
which gives the claimed amortized recourse tradeoff according to \eqref{eq:recourse-is-d}.


==> macros.tex <==
\usepackage{typearea}
\usepackage{setspace}

\usepackage{fullpage}

\usepackage{comment} 
\usepackage{bbm}
\usepackage{framed} 
\usepackage{url} 
\usepackage{complexity}
\usepackage{booktabs}
\usepackage{amsmath,amssymb}
\usepackage{float}

\usepackage{amsthm}
\usepackage{thmtools} 
\usepackage{thm-restate}
\usepackage{nicefrac}
\usepackage{calc}
\usepackage{enumerate}
\usepackage{enumitem}
\usepackage[usenames,dvipsnames]{xcolor}
%\usepackage{algorithm}

\usepackage[ruled,vlined,linesnumbered]{algorithm2e}
\usepackage{forloop}

\usepackage{graphicx}
\usepackage[font=footnotesize,labelfont=bf]{subcaption}
\usepackage[font=footnotesize,labelfont=bf]{caption}
\usepackage[nobreak=true]{mdframed}
\usepackage{appendix}
\usepackage[noend]{algpseudocode}
\usepackage[colorinlistoftodos]{todonotes}
\usepackage{xr}
\usepackage{array}
\usepackage{xspace}
\definecolor{ForestGreen}{rgb}{0.1333,0.5451,0.1333}
\definecolor{DarkRed}{rgb}{0.8,0,0}
\definecolor{Red}{rgb}{1,0,0}
\usepackage[linktocpage=true,
pagebackref=true,colorlinks,
linkcolor=DarkRed,citecolor=ForestGreen,
bookmarks,bookmarksopen,bookmarksnumbered]{hyperref}

\renewcommand\backrefpagesname{\(\rightarrow\) cited on page}
\renewcommand\backref{\backrefpagesname\ }

\usepackage[capitalise]{cleveref}
\crefrangelabelformat{enumi}{#3#1#4--#5#2#6}
\usepackage{parskip}
\usepackage{chngcntr}
\usepackage{mathtools,stackengine}
\usepackage{multirow}

\stackMath
\newcommand{\stackGeq}[1]{%
	\setbox0=\hbox{${}\mathrel{\stackon[-1pt]{\geq}{\scriptstyle\text{#1\strut}}}{}$}
	\xdef\tmpwd{\dimexpr\the\wd0\relax}
	\kern.5\tmpwd\mathclap{\box0}&\kern.5\tmpwd
}

\usepackage{nameref}
% folowing  must be in this order

\usepackage{tikz}
\usetikzlibrary{patterns}

% \makeatletter
% \setlength{\parindent}{0pt}
% \addtolength{\partopsep}{-2mm}
% \setlength{\parskip}{5pt plus 1pt}
% \addtolength{\abovedisplayskip}{-10mm}
% \addtolength{\textheight}{35pt}
% \addtolength{\footskip}{-20pt}
% \makeatother
\allowdisplaybreaks

\DeclareMathOperator*{\Ber}{Ber}
\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\argmax}{argmax}
\let\polylog\relax
\DeclareMathOperator*{\polylog}{polylog}
\DeclareMathOperator*{\med}{med}
\DeclareMathOperator*{\RowSpan}{RowSpan}
\DeclareMathOperator*{\ColSpan}{ColSpan}
\DeclareMathOperator*{\Exp}{Exp}
\DeclareMathOperator*{\expectation}{\mathbb{E}}
\let\poly\relax
\DeclareMathOperator*{\poly}{poly}
\DeclareMathOperator*{\cov}{cov}
\DeclareMathOperator*{\probability}{\mathbb{P}}

\newcommand{\one}{{\sc Type 1}\xspace}
\newcommand{\two}{{\sc Type 2}\xspace}
\newcommand{\three}{{\sc Type 3}\xspace}
\newcommand{\four}{{\sc Type 4}\xspace}

\newcommand{\eat}[1]{}

\newcommand{\tO}{\tilde{O}}

\newcommand{\ins}{{\tt insert}}

\newcommand\singleangle[1]{\langle #1 \rangle}
\newcommand\doubleangle[1]{\langle \langle #1 \rangle \rangle}
\newcommand\lcm{\text{lcm}}
\newcommand\rank{\text{ rank }}
\newcommand{\vol}{\text{vol}}
\renewcommand\R{\mathbb{R}}
\let\U\relax
\newcommand{\U}{\mathcal{U}}
\newcommand\Z{\mathbb{Z}}
\renewcommand\C{\mathcal{C}}
\renewcommand\P{\mathcal{P}}
\newcommand\mff{\mathfrak{F}}
\newcommand\mfI{\mathfrak{I}}
\newcommand\nnz{\text{nnz}}
\newcommand\eps{\varepsilon}
\newcommand\sign[1]{\text{sgn}\left(#1\right)}
\newcommand\norm[1]{\left\| #1 \right\|}
\newcommand\fnorm[1]{\norm {#1 }_F}
\newcommand\inorm[1]{\norm {#1 }_\infty}
\newcommand\pnorm[2]{\norm {#1 }_{#2}}
\newcommand\partwrt[2]{\frac{\partial #1}{\partial #2}}
\newcommand\sgn{\text{sgn}}
\newcommand\Id{\mathcal{I}}
\newcommand\unvrs{\mathcal{N}}
\newcommand\abs[1]{\lvert #1 \rvert}
\newcommand{\expect}{\expectation\expectarg}
\DeclarePairedDelimiterX{\expectarg}[1]{[}{]}{%
	\ifnum\currentgrouptype=16 \else\begingroup\fi
	\activatebar#1
	\ifnum\currentgrouptype=16 \else\endgroup\fi
}

\newcommand\tbuy{\mathcal{T}_{\text{cust}}}
\newcommand\tsell{\mathcal{T}_{\text{supp}}}

\newcommand\primy{\overline{y}}
\newcommand\primz{\overline{z}}
\newcommand\primr{\overline{r}}

\newcommand\dualx{\overline{x}}
\newcommand\duall{\overline{\ell}}
\newcommand\duala{\overline{\alpha}}
\newcommand\dualb{\overline{\beta}}

\newcommand\vt{v}
\newcommand\vmax{v_{\max}}


\newcommand{\expectover}[1]{\expectation_{#1}\expectarg}

\newcommand{\niceset}{\nicesetarg}
\DeclarePairedDelimiterX{\nicesetarg}[1]{\{}{\}}{%
	\ifnum\currentgrouptype=16 \else\begingroup\fi
	\activatebar#1
	\ifnum\currentgrouptype=16 \else\endgroup\fi
}

\newcommand{\innermid}{\nonscript\;\delimsize\vert\nonscript\;}
\newcommand{\activatebar}{%
	\begingroup\lccode`\~=`\|
	\lowercase{\endgroup\let~}\innermid 
	\mathcode`|=\string"8000
}

\newcommand\prob[1]{\probability\left( #1 \right)}
\newcommand\probarg[2]{\probability_{#2}\left( #1 \right)}
\newcommand\mutcov{\mathcal{I}}
\newcommand\opt{\mathsf{opt}\xspace}
\newcommand\alg{\mathsf{alg}\xspace}
\newcommand\sse{\subseteq}

\counterwithin{equation}{section}

\newcommand{\Continue}{\textbf{continue}\xspace}
%\newcommand{\ForEach}{\textbf{for each}\xspace}
\newcommand{\Break}{\textbf{break}\xspace}

\newcommand\alginput[1]{\hspace*{\algorithmicindent} \textbf{Input:} #1}
\newcommand\algoutput[1]{\hspace*{\algorithmicindent} \textbf{Output:} #1}
\usepackage{eqparbox}
\renewcommand{\algorithmiccomment}[1]{\hfill\eqparbox{COMMENT}{// #1}}

\def\nonl#1{{\def\alglinenumber##1{}\State #1}\addtocounter{ALG@line}{-1}}

\newcommand\fmin{f_{\min}}
\newcommand\fmax{f_{\max}}
\newcommand\gmin{g_{\min}}
\newcommand\gmax{g_{\max}}

\newcommand\cmin{c_{\min}}
\newcommand\cmax{c_{\max}}
\newcommand{\ov}[1]{{\color{cyan}OV: #1}\marginpar{$\star\star$}}
\newcommand{\iancomment}[1]{{\color{cyan}IAN: #1}\marginpar{$\star\star$}}
\newcommand\KL[2]{\textsc{KL}\left(#1 \mid \mid #2\right)}
\newcommand\wKL[2]{\textsc{KL}_w\left(#1 \mid \mid #2\right)}

\newcommand\Ell{\mathcal{L}}

\newcommand\mst{\textsc{MinimumSpanningTree}\xspace}
\newcommand\mstt{\textsc{MinimumSteinerTree}\xspace}
\newcommand\setcov{\textsc{SetCover}\xspace}
\newcommand\loadbal{\textsc{LoadBalancing}\xspace}
\newcommand\matching{\textsc{Matching}\xspace}
\newcommand\hitset{\textsc{HittingSet}\xspace}
\newcommand\chasehyp{\textsc{ChasingHalfspaces}\xspace}
\newcommand\hvc{\textsc{HypergraphVertexCover}\xspace}
\newcommand\subcov{\textsc{SubmodularCover}\xspace}
\renewcommand\SAT{\textsc{SAT}\xspace}

\theoremstyle{plain}
\usepackage{aliascnt}

\newtheorem{theorem}{Theorem}[section]
\newtheorem{definition}[theorem]{Definition}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{fact}[theorem]{Fact}
\newtheorem{observation}[theorem]{Observation}

\newaliascnt{claim}{theorem}
\newtheorem{claim}{Claim}
\aliascntresetthe{claim}
\crefname{claim}{claim}{claims}
\Crefname{claim}{Claim}{Claims}

\newtheorem{subclaim}[theorem]{Subclaim}
\newtheorem{example}[theorem]{Example}
\newtheorem{construction}[theorem]{Construction}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{reduction}[theorem]{Reduction}
\newtheorem{invariant}{Invariant}
\newtheorem{extension}[theorem]{Extension}
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{remark}[theorem]{Remark}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%% ADD INDENTATION TO MULTILINE STATEMENTS %%%%%%%%%%%%%%

\newlength{\continueindent}
\setlength{\continueindent}{2em}
\usepackage{etoolbox}
\makeatletter
\newcommand*{\ALG@customparshape}{\parshape 2 \leftmargin \linewidth \dimexpr\ALG@tlm+\continueindent\relax \dimexpr\linewidth+\leftmargin-\ALG@tlm-\continueindent\relax}
\apptocmd{\ALG@beginblock}{\ALG@customparshape}{}{\errmessage{failed to patch}}
\makeatother

\makeatletter
\def\thm@space@setup{%
	\thm@preskip=\parskip \thm@postskip=0pt
}
\makeatother

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%% ADD VERTICAL LINES TO CODE BLOCKS %%%%%%%%%%%%%%%%%%%

\usepackage{etoolbox}
\usepackage{tikz}
\usetikzlibrary{tikzmark}
\usetikzlibrary{calc}

\errorcontextlines\maxdimen

% begin vertical rule patch for algorithmicx (http://tex.stackexchange.com/questions/144840/vertical-loop-block-lines-in-algorithmicx-with-noend-option)
% note that some of the packages above are also needed
\newcommand{\ALGtikzmarkcolor}{black}% customise this, if you want
\newcommand{\ALGtikzmarkextraindent}{4pt}% customise this, if you want
\newcommand{\ALGtikzmarkverticaloffsetstart}{-.5ex}% customise this, if you want
\newcommand{\ALGtikzmarkverticaloffsetend}{-.5ex}% customise this, if you want
\makeatletter
\newcounter{ALG@tikzmark@tempcnta}

\newcommand\ALG@tikzmark@start{%
	\global\let\ALG@tikzmark@last\ALG@tikzmark@starttext%
	\expandafter\edef\csname ALG@tikzmark@\theALG@nested\endcsname{\theALG@tikzmark@tempcnta}%
	\tikzmark{ALG@tikzmark@start@\csname ALG@tikzmark@\theALG@nested\endcsname}%
	\addtocounter{ALG@tikzmark@tempcnta}{1}%
}

\def\ALG@tikzmark@starttext{start}
\newcommand\ALG@tikzmark@end{%
	\ifx\ALG@tikzmark@last\ALG@tikzmark@starttext
	% ignore this, the block was opened then closed directly without any other blocks in between (so just a \State basically)
	% don't draw a vertical line here
	\else
	\tikzmark{ALG@tikzmark@end@\csname ALG@tikzmark@\theALG@nested\endcsname}%
	\tikz[overlay,remember picture] \draw[\ALGtikzmarkcolor] let \p{S}=($(pic cs:ALG@tikzmark@start@\csname ALG@tikzmark@\theALG@nested\endcsname)+(\ALGtikzmarkextraindent,\ALGtikzmarkverticaloffsetstart)$), \p{E}=($(pic cs:ALG@tikzmark@end@\csname ALG@tikzmark@\theALG@nested\endcsname)+(\ALGtikzmarkextraindent,\ALGtikzmarkverticaloffsetend)$) in (\x{S},\y{S})--(\x{S},\y{E});%
	\fi
	\gdef\ALG@tikzmark@last{end}%
}

% the following line injects our new tikzmarking code
\apptocmd{\ALG@beginblock}{\ALG@tikzmark@start}{}{\errmessage{failed to patch}}
\pretocmd{\ALG@endblock}{\ALG@tikzmark@end}{}{\errmessage{failed to patch}}
\makeatother
% end vertical rule patch for algorithmicx

\algblock[with]{With}{EndWith}
\algblockdefx[With]{With}{EndWith}%
[1]{\textbf{with} #1 \textbf{do}}%
{}

\makeatletter
\ifthenelse{\equal{\ALG@noend}{t}}%
{\algtext*{EndWith}}
{}%
\makeatother


\global\long\def\all{\textsc{all}}
\global\long\def\NULL{\texttt{null}}
\global\long\def\inner#1#2{\left\langle #1,#2\right\rangle }
\global\long\def\onevec{\vec{1}}

\newcommand{\dd}[1]{{\color{purple}DD: #1}\marginpar{$\star\star$}}

\newcommand{\nb}[1]{{\color{red}NB: #1}\marginpar{$\star\star$}}

\newcommand{\hx}{\hat{x}}
\newcommand{\cE}{{\cal E}}



==> new_ADST_files/ADST_size.tex <==
We next establish the size bounds needed for the
reconstruction of an \adst. We first bound the number
of cells it can contain, and then show that these
cells can always be accommodated by a single \dst\
of the same level.

\begin{claim}
\label{cl:adst-size}
For every $i<d$, an $i$-level \adst\ contains at
most $2^i$ cells after every completed update.
\end{claim}

\begin{proof}
Each invocation of \resort$(i+1)$ leaves its
level-$i$ auxiliary \adst\ empty. Each subsequent
deletion--insertion pair can increase its size by
at most one cell, and \resort$(i+1)$ is invoked
again after at most $2^i$ such updates.

Since rebuilding within the auxiliary \adst\
does not increase its total size, the claim follows.
\end{proof}

To ensure that reconstruction is possible, we also
need to verify that the Block Sizes invariant allows
a clean \dst\ to contain sufficiently many elements.

\begin{claim}
\label{cl:dst-capacity}
For every $i\ge 1$, a clean $i$-level \dst\
can be constructed from any $N\le 12\cdot 2^i$
elements while satisfying all structural invariants.
\end{claim}

\begin{proof}
We prove the claim by induction on $i$.
For $i=1$, the \dst\ is a sorted array of at most
$24$ cells.

Suppose $i>1$, and let $q=2^{i-1}$.
If $N\le 11q$, we construct a single block,
which is feasible by induction.

Otherwise, we construct three blocks according
to the rebuilding rule. The middle block contains
$q$ cells, the last contains
\[
    L=\max\left\{
        8q,\left\lceil\frac{N-q}{2}\right\rceil
    \right\},
\]
and the first contains $F=N-q-L$ cells.

Since $11q<N\le24q$, we have
\[
    2q\le F<12q,
    \qquad
    8q\le L<12q.
\]
Thus, the block sizes satisfy the required bounds,
and their recursive sections can be constructed
by induction. Placing the elements in sorted
order and leaving all transfer sections empty
ensures the ordering invariants.
\end{proof}

We can now fix the recursion depth as
\[
    d=\max\left\{
        1,\left\lceil\log_2(n/12)\right\rceil
    \right\}.
\]
Since $n\le12\cdot2^d$, the top-level \adst\
can be reconstructed into a clean $d$-level \dst.
By \cref{cl:adst-size,cl:dst-capacity}, every
lower-level \adst\ can likewise be reconstructed
into a clean \dst\ of its level. Hence, all
invocations of \resort\ are feasible.


==> new_ADST_files/two-level-illustration.tex <==
% Also uses the operation macro \swaphole defined in the main paper.
\begin{figure}[t]
\centering
\resizebox{0.95\linewidth}{!}{%
\begin{tikzpicture}[
  x=1cm,y=1cm,
  every node/.style={font=\small},
  original/.style={fill=blue!9,draw=black!45,line width=.4pt},
  transferred/.style={fill=orange!19,draw=black!45,line width=.4pt},
  hole/.style={draw=red!80!black,line width=1.05pt},
  donor/.style={draw=green!40!black,line width=1.0pt},
  action/.style={-{Latex[length=2mm]},black!65,line width=.8pt},
  block/.style={draw=black!65,line width=.7pt},
  stagelabel/.style={font=\footnotesize,anchor=east,align=right},
  steptext/.style={font=\footnotesize,anchor=west}
]

% Cell positions are fixed throughout the illustration.
\newcommand{\origcell}[3]{%
  \path[original] (#1,#2) rectangle ++(.70,.60);
  \node at ({#1+.35},{#2+.30}) {$#3$};%
}
\newcommand{\transcell}[3]{%
  \path[transferred] (#1,#2) rectangle ++(.70,.60);
  \node at ({#1+.35},{#2+.30}) {$#3$};%
}
\newcommand{\ocell}[2]{%
  \path[original] (#1,#2) rectangle ++(.70,.60);
  \path[hole] (#1,#2) rectangle ++(.70,.60);
  \node[red!80!black] at ({#1+.35},{#2+.30}) {$\circ$};%
}
\newcommand{\tcell}[2]{%
  \path[transferred] (#1,#2) rectangle ++(.70,.60);
  \path[hole] (#1,#2) rectangle ++(.70,.60);
  \node[red!80!black] at ({#1+.35},{#2+.30}) {$\circ$};%
}
\newcommand{\highlightcell}[2]{%
  \path[donor] (#1,#2) rectangle ++(.70,.60);%
}
\newcommand{\outlines}[1]{%
  \draw[block] (0,#1) rectangle (1.40,{#1+.60});
  \draw[block] (1.68,#1) rectangle (5.18,{#1+.60});
  \draw[block] (5.46,#1) rectangle (8.26,{#1+.60});
  \draw[block] (8.54,#1) rectangle (9.94,{#1+.60});%
}
\newcommand{\firstandlast}[2]{%
  \origcell{0}{#1}{1}\origcell{.70}{#1}{2}
  #2%
}
\newcommand{\stagearrow}[2]{%
  \draw[action] (.48,{#1-.12}) -- (.48,{#1-.88});
  \node[steptext] at (1.12,{#1-.50}) {#2};%
}

% First-row block and section labels.
\foreach \x/\name in {.70/B_1,3.43/B_2,6.86/B_3,9.24/B_4}{
    \node[font=\small\bfseries] at (\x,8.28) {$\name$};
}
\node[font=\scriptsize,text=orange!65!black] at (2.03,7.93) {$T_2$};
\node[font=\scriptsize,text=blue!65!black] at (3.78,7.93) {$O_2$};
\node[font=\scriptsize,text=orange!65!black] at (5.81,7.93) {$T_3$};
\node[font=\scriptsize,text=blue!65!black] at (7.21,7.93) {$O_3$};

% State 0: before deletion.
\node[stagelabel] at (-.25,7.41) {Before deletion};
\firstandlast{7.11}{%
  \transcell{1.68}{7.11}{8}
  \origcell{2.38}{7.11}{3}\origcell{3.08}{7.11}{4}
  \origcell{3.78}{7.11}{5}\origcell{4.48}{7.11}{6}
  \transcell{5.46}{7.11}{12}
  \origcell{6.16}{7.11}{9}\origcell{6.86}{7.11}{10}\origcell{7.56}{7.11}{11}
  \origcell{8.54}{7.11}{13}\origcell{9.24}{7.11}{14}
}
\outlines{7.11}
\stagearrow{7.11}{Delete $4$ and shift $5,6$ one position left}

% State 1: hole at end of O2.
\node[stagelabel] at (-.25,5.81) {Hole at end of $O_2$};
\firstandlast{5.51}{%
  \transcell{1.68}{5.51}{8}
  \origcell{2.38}{5.51}{3}\origcell{3.08}{5.51}{5}\origcell{3.78}{5.51}{6}\ocell{4.48}{5.51}
  \transcell{5.46}{5.51}{12}
  \origcell{6.16}{5.51}{9}\origcell{6.86}{5.51}{10}\origcell{7.56}{5.51}{11}
  \origcell{8.54}{5.51}{13}\origcell{9.24}{5.51}{14}
}
\highlightcell{1.68}{5.51}
\outlines{5.51}
\stagearrow{5.51}{Move $8=\min T_2$ into the hole in $O_2$}

% State 2: hole in T2.
\node[stagelabel] at (-.25,4.21) {Hole in $T_2$};
\firstandlast{3.91}{%
  \tcell{1.68}{3.91}
  \origcell{2.38}{3.91}{3}\origcell{3.08}{3.91}{5}\origcell{3.78}{3.91}{6}\origcell{4.48}{3.91}{8}
  \transcell{5.46}{3.91}{12}
  \origcell{6.16}{3.91}{9}\origcell{6.86}{3.91}{10}\origcell{7.56}{3.91}{11}
  \origcell{8.54}{3.91}{13}\origcell{9.24}{3.91}{14}
}
\highlightcell{6.16}{3.91}
\outlines{3.91}
\stagearrow{3.91}{Move $9=\min O_3$ into $T_2$; move the hole from $O_3$ to $T_3$}

% State 3: hole in T3.
\node[stagelabel] at (-.25,2.61) {Hole in $T_3$};
\firstandlast{2.31}{%
  \transcell{1.68}{2.31}{9}
  \origcell{2.38}{2.31}{3}\origcell{3.08}{2.31}{5}\origcell{3.78}{2.31}{6}\origcell{4.48}{2.31}{8}
  \transcell{5.46}{2.31}{12}\tcell{6.16}{2.31}
  \origcell{6.86}{2.31}{10}\origcell{7.56}{2.31}{11}
  \origcell{8.54}{2.31}{13}\origcell{9.24}{2.31}{14}
}
\highlightcell{8.54}{2.31}
\outlines{2.31}
\stagearrow{2.31}{Move $13=\min B_4$ into $T_3$}

% State 4 (new): after transferring 13, hole is at start of last block.
\node[stagelabel] at (-.25,1.01) {Hole in $B_4$};
\firstandlast{.71}{%
  \transcell{1.68}{.71}{9}
  \origcell{2.38}{.71}{3}\origcell{3.08}{.71}{5}\origcell{3.78}{.71}{6}\origcell{4.48}{.71}{8}
  \transcell{5.46}{.71}{12}\transcell{6.16}{.71}{13}
  \origcell{6.86}{.71}{10}\origcell{7.56}{.71}{11}
  \ocell{8.54}{.71}\origcell{9.24}{.71}{14}
}
\highlightcell{9.24}{.71}
\outlines{.71}
\stagearrow{.71}{Shift $14$ one position left}

% State 5 (new): final hole at the end of last block.
\node[stagelabel] at (-.25,-.59) {Final hole};
\firstandlast{-.89}{%
  \transcell{1.68}{-.89}{9}
  \origcell{2.38}{-.89}{3}\origcell{3.08}{-.89}{5}\origcell{3.78}{-.89}{6}\origcell{4.48}{-.89}{8}
  \transcell{5.46}{-.89}{12}\transcell{6.16}{-.89}{13}
  \origcell{6.86}{-.89}{10}\origcell{7.56}{-.89}{11}
  \origcell{8.54}{-.89}{14}\ocell{9.24}{-.89}
}
\outlines{-.89}

% Legend.
\node[font=\footnotesize,anchor=west,text=black!75] at (0,-1.55)
   {\textcolor{blue!65!black}{Blue}: original\qquad
    \textcolor{orange!70!black}{Orange}: transfer\qquad
    \textcolor{green!45!black}{Green outline}: next donor\qquad
    \textcolor{red!75!black}{Red outline}: hole};
\end{tikzpicture}%
}
\caption{Deleting $4$ in the simplified two-level structure.
The hole first reaches the end of $O_2$, is filled by $8$ from $T_2$,
and then advances by borrowing $9$ and $13$ from successive blocks.
The boundary change between $T$ and $O$ moves no elements. 
The final shift of $14$
leaves the hole at the end of the array.}
\label{fig:dst-example}
\end{figure}

==> other_related_works.tex <==
\paragraph{Online Sorting.} The online sorting problem was originally motivated by online packing problems for convex objects, including online strip packing~\cite{BakerS83,CsirikW97,HanIYZ07,YeHZ09,GerlachHK26} and online rectangle bin packing~\cite{CoppersmithR89,Galambos91,Vliet92,GalambosV94,CsirikFL93,CsirikV93,SeidenS03,HanCTZZ11}. It can also be viewed as an online traveling salesman problem on the line metric, which naturally generalizes to arbitrary metric spaces. Abrahamsen {\em et al.}~\cite{AbrahamsenB0K024} established tight $\Theta(\log n)$ bounds for the uniform metric and posed the general metric case as an open problem. This was recently resolved by Bertram~\cite{Bertram25}, who obtained an $O(\sqrt n)$-competitive algorithm for arbitrary metric spaces. Given the $\Omega(\sqrt n)$ lower bound on the line metric, this bound is asymptotically tight.



% \paragraph{Online List Labeling.} Variants of online list labeling include online house numbering~\cite{devanny2017}, workload-adaptive algorithms~\cite{benderhu2007,bfgkm2017}, and learning-augmented list labeling~\cite{mccauley2023}. The problem also underlies numerous data structures and algorithms, including cache-oblivious B-trees and dictionaries~\cite{bcdf2000,bfj2002,bdiw2002,bfgk2005,bfk2006,bender2016tods,bcdf2002scan}, packed-memory arrays~\cite{raman1999,deleo2019icde,deleo2019grades,pandey2021terrace,wheatman2021parallel}, insertion sort~\cite{bfm2006}, sparsification for dynamic graph algorithms~\cite{egin1997}, online topological ordering~\cite{katriel2006}, fault-tolerant data structures~\cite{aumannbender1996}, the distributed controller problem~\cite{kormankutten2007,emekkorman2011}, and predecessor queries over general alphabets~\cite{kopelowitz2012}.


% \eat{
% \paragraph{Online List-Labeling.}
% Itai, Konheim, and Rodeh~\cite{itai1981} introduced the online list-labeling problem, also called the file-maintenance problem, and gave an algorithm with $O(\log^2 n)$ amortized cost per operation in linear space, $m=(1+\Theta(1))n$. Willard~\cite{willard1982, willard1986,willard1992} deamortized this bound, giving $O(\log^2 n)$ worst-case cost per operation in the same space. Galperin and Rivest~\cite{galperinrivest1993} show that scapegoat trees achieve the same worst-case bound.

% In the polynomial-space regime, $m=n^{1+\Omega(1)}$, Dietz and Sleator~\cite{dietz1987} give an $O(\log n)$ amortized algorithm, which also yields $O(1)$ amortized updates with $O(1)$-time queries for the related order-maintenance problem posed by Dietz~\cite{dietz1982}. Bender, Cole, Demaine, Farach-Colton, and Zito~\cite{bcdfz2002} give simplified algorithms with the same guarantees. This line of work underlies the classical persistence technique of Driscoll, Sarnak, Sleator, and Tarjan~\cite{dsst1989}.

% On the lower-bound side, Dietz and Zhang~\cite{dietz1990} prove an $\Omega(\log^2 n)$ bound for smooth algorithms (those that rebalance by spreading items out evenly) in linear space. Dietz, Seiferas, and Zhang~\cite{dietz2004,zhang1993} prove an $\Omega(n\log n)$ bound for arbitrary deterministic algorithms in polynomial space, matching~\cite{dietz1987}. Bul\'anek, Kouck\'y, and Saks~\cite{bulanek2012,bulanek2015} extend the $\Omega(\log^2 n)$ bound to all deterministic algorithms in linear space, matching~\cite{itai1981} and settling the deterministic complexity of the problem.

% For randomized algorithms, Bul\'anek, Kouck\'y, and Saks~\cite{bulanek2013} prove a matching $\Omega(\log n)$ bound in polynomial space, settling that regime. In linear space, however, the best known randomized lower bound remained only $\Omega(\log n)$, a full $\log n$ factor below the deterministic $\Omega(\log^2 n)$ bound; Saks~\cite{saks2018} surveys this gap as the central open question in the area. Babka, Bul\'anek, \v{C}un\'at, Kouck\'y, and Saks~\cite{babka2012,babka2019} extend the lower-bound landscape to superpolynomial and exponentially large label spaces.

% The gap was closed using ideas from the history-independent data structures literature~\cite{naorteague2001,hartline2002,bender2016pods}, whose data structures' internal state depends only on the current set of stored elements rather than on operation history. Bender, Conway, Farach-Colton, Koml\'os, Kuszmaul, and Wein~\cite{bender2024siam} use this property to give a randomized algorithm with $O(\log^{3/2} n)$ expected amortized cost, the first improvement over $O(\log^2 n)$ in forty-one years.

% Bender, Conway, Farach-Colton, Koml\'os, and Kuszmaul~\cite{bender2024layered} give a compositional technique that simultaneously achieves $O(\log n)$ expected cost on favorable workloads, $O(\log^{3/2}n)$ expected cost in general, and $O(\log^2 n)$ worst-case cost, combining the best known guarantees along all three axes. Bender, Conway, Farach-Colton, Koml\'os, Kouck\'y, Kuszmaul, and Saks~\cite{bender2024nearly} then give the See-Saw algorithm, achieving $O(\log n \cdot \mathrm{polyloglog}\,n)$ amortized expected cost, within a sub-polynomial factor of the $\Omega(\log n)$ lower bound. Bender, Farach-Colton, Goodrich, and Koml\'os~\cite{bender2024partitioning} generalize the underlying history-independence ideas to a related dynamic-partitioning problem. Closing the remaining gap to $\Omega(\log n)$ remains open.

% Variants of the problem include the online house-numbering problem of Devanny, Fineman, Goodrich, and Kopelowitz~\cite{devanny2017}, which minimizes the maximum label gap rather than total relabeling cost, and workload-adaptive algorithms~\cite{benderhu2007,bfgkm2017} that retain worst-case guarantees while performing better on structured workloads.

% Learning-augmented list labeling, motivated by learned index structures~\cite{kraska2018}, is introduced by McCauley, Moseley, Niaparast, and Singh~\cite{mccauley2023}, who give an algorithm whose cost degrades gracefully with the error of a predicted rank while matching the best known worst-case bound when predictions are wrong; this algorithm composes with the bounds of~\cite{bender2024layered} above.

% List labeling underlies cache-oblivious B-trees and dictionaries~\cite{bcdf2000,bfj2002,bdiw2002,bfgk2005,bfk2006,bender2016tods,bcdf2002scan}; packed-memory arrays used in database and graph systems~\cite{raman1999,deleo2019icde,deleo2019grades,pandey2021terrace,wheatman2021parallel}; $O(n\log n)$ insertion sort~\cite{bfm2006}; sparsification for dynamic graph algorithms~\cite{egin1997}; online topological ordering~\cite{katriel2006}; fault-tolerant data structures~\cite{aumannbender1996}; the distributed controller problem~\cite{kormankutten2007,emekkorman2011}; and predecessor queries over general alphabets~\cite{kopelowitz2012}.




